Spoke-Darts for High-Dimensional Blue-Noise Sampling

Blue noise sampling has proved useful for many graphics applications, but remains underexplored in high-dimensional spaces due to the difficulty of generating distributions and proving properties about them. We present a blue noise sampling method with good quality and performance across different dimensions. The method, spoke-dart sampling, shoots rays from prior samples and selects samples from these rays. It combines the advantages of two major high-dimensional sampling methods: the locality of advancing front with the dimensionality-reduction of hyperplanes, specifically line sampling. We prove that the output sampling is saturated with high probability, with bounds on distances between pairs of samples and between any domain point and its nearest sample. We demonstrate spoke-dart applications for approximate Delaunay graph construction, global optimization, and robotic motion planning. Both the blue-noise quality of the output distribution and the adaptability of the intermediate processes of our method are useful in these applications.

==> Spoke_MPS_demo_fig.tex <==
\begin{figure}[tbh]
\centering
     \includegraphics[width=\columnwidth]{figs/overview_hid}
 \caption{ \Spokedart s. We throw a line (blue) through an extant sample (red). The line is clipped by prior sample disks (green) and a new sample (cyan) is added on a remaining segment.}
 \label{fig:spoke_mps_demo}
\end{figure}


==> ack-my.tex <==
\section*{Acknowledgements}
%We are grateful to Gamito and Maddock for freely providing their software.
%
<<<<<<< HEAD
We thank Robert Bridson for making his software~\cite{bridson:code} available.
We thank the authors of PSA for making their software available.
We thank the reviewers for their helpful feedback and suggestions.

This material is based upon work supported by the U.S. Department of Energy, Office of Science, Office of Advanced Scientific Computing Research (ASCR), Applied Mathematics Program. Sandia National Laboratories is a multi-program laboratory managed and operated by Sandia Corporation, a wholly owned subsidiary of Lockheed Martin Corporation, for the U.S. Department of Energy?s National Nuclear Security Administration under contract DE-AC04-94AL85000.

=======
We thank Robert Bridson and the authors of PSA for making their software available, and the reviewers for their helpful feedback and suggestions.
Sandia National Laboratories is a multi-program laboratory managed and operated by Sandia Corporation, a wholly owned subsidiary of Lockheed Martin Corporation, for the U.S. Department of Energy's National Nuclear Security Administration under contract DE-AC04-94AL85000.
>>>>>>> 42b038b56bb7f4ac32754a8ebad99ca34ad29d1b


==> algorithm_issues.tex <==
\subsection{\nothing{Sampling }Algorithms}
\label{sec:algorithm_issues}

\pargrph{High dimensional neighbor finding}
%
%The curse-of-dimensionality refers to the difficulty of obtaining efficient data-structures and algorithms in high dimensions.
%The goal is to avoid time and memory complexities higher than polynomial.
%
Detecting nearby samples is a key step for random blue noise methods.%\liyi{(February 6, 2016) The percentage sign at the end of a line can help prevent unnecessary breaks from the next, such as a footnote.}%liyi
\footnote{We consider pseudo-random patterns such as low discrepancy sequences as out of scope.}
%The efficiency of random blue noise algorithms appears to be limited by neighbor finding for the foreseeable future.
This is fundamentally difficult, because the number of neighbors depends exponentially on $\dimnumber$.
%Specifically, the number of small balls that can fit within a larger ball grows exponentially with dimension $\dimnumber$.
%, related to the mathematical \emacsquote{kissing number.} 
Many popular low-dimensional algorithms make this worse by introducing steps or datastructures exponential in  $\dimnumber.$
For example, facillitating searches with a background grid of cubes is popular in low dimensions.
It is ``constant time and size'' for fixed dimension but $2^{O(d)}.$

Neighborhood queries in high dimensions is a longstanding and active research topic in computational geometry~\cite{Samet:2005:FMM,proximitysurvey,Miller:2013:FAW}.
Many of the best methods are based on $k$-d trees~\cite{Samet:2005:FMM}.
A key advantage is $k$-d trees require only \emph{linear} memory, $\dOmemory.$
%The problem is 
%not the complexity of the datastructure, but 
Time is $O(\samplenumber \log \samplenumber)$ for low dimensions.
Performance degrades gracefully as the dimension increases, approaching the time for exhaustive search. %, \emph{all-distances}.
The good news is that this is only linear in the output size $n$, regardless of dimension.
Generating high dimensional blue noise in linear $O(dn)$ time would be ideal, but $O(dn^2)$ is about the best one can hope for.
%, where $n$ is the output size (number of accepted samples).
\footnote{$k$-d tree query time is $O(n^{1-1/d} + N)$, where $N$ is the number of nearby points and $n$ is the total number of points. The query is typically done $n$ times, and it takes $d$ time to compute the distance between two points, leading to $O(\dimnumber \samplenumber^2)$. The time to create the tree is dominated by this.}
%Memory is more important than time.
%A high time complexity means we must wait for an answer. 
%A high memory complexity means we will get no answer.

%So, while background grids work extremely well in low dimensions, they become intractable as the dimension increases. 
%
%
%For fixed dimensions, this gives $O(\samplenumber \log \samplenumber)$ complexity.
%(One could obtain $O(\samplenumber)$ using a background grid.)
%For high dimensions, the query time of the tree degrades this to $O(\dimnumber \samplenumber^2).$ 


\pargrph{Sample elimination}
Yuksel~\shortcite{10.1111:cgf.12538} generates dense white noise, then eliminates some points based on proximity.
% to other points.
%, leaving a distribution with blue noise. 
% note: proximity metric is complicated
This supports progressive sampling, and the user can specify the exact number of sample points.
The runtime scales well with dimension, and efficient neighbor-finding is the limiting step. % as the dimension increases. %, leading to $O(d n^2)$ runtime.
% note: they do 16,000 points in 256 dimensions. I don't think this is for periodic domains. They don't discuss periodic vs aperiodic domains at all.
% its not clear what happens when a point is close to multiple periodic copies of a point. Since they don't do any geometric primitives, this might be OK.
Unfortunately, there are no guarantees of well-spacedness, neither a lower bound on sample separation, nor an upper bound on domain-to-sample distance.

 
% Our interpretation is that \bridsonmethod\ provides no guarantee of saturation for any rejection limit.
% true, but sufficient to say there is no published bound. 
%
% our proof method \Cref{sec:boundproofs} relies on the surface area does not provide one.
% We collect the void boundary surface area and say that the void is smaller than a sphere with the same surface area.
% Here, if we collect the "boundary volume" into a volume, not sure how to proceed from there ...


\pargrph{Local sampling for saturation}
One way to guarantee local saturation is to construct the unsaturated regions for local dart throwing. 
Jones~\shortcite{Jones:2005:EGPDS} uses Delaunay triangles.
Many use background grids~\cite{Dunbar:2006:PDS}. This approach is fundamentally limited to low dimensions.
E.g.\ Simple MPS was demonstrated on periodic domains up to 3D, and aperiodic up to 6D~\cite{Ebeida:2012:SAM}.

\pargrph{Step blue noise through optimization}
Most step blue noise algorithms require compute-intensive optimization as a post-process of an initial distribution \cite{Heck:2013:BNS,Spencer:2013:PPR:2421636.2421643,Zhou:2012:PSGNS,Oztireli:2012:ASP,Jiang:2015:BNS}.
The exceptions include a method based on refining particular tile patterns, which appears fundamentally 2D \cite{Wachtel:2014:FTA:2601097.2601107}.
Two-Radii MPS produces step blue noise directly from a background grid~\cite{Mitchell:2012:VRPD}.




\pargrph{Advancing front}
%
Advancing front methods were initially proposed for meshing \cite{firstspheremesh,Li99biting:advancing,fastspherepacking} and later adopted for sampling in graphics \cite{Jones:2005:EGPDS,Dunbar:2006:PDS,Bridson:2007:FPD}.
The basic idea is to draw new samples from regions around the existing samples (the front) and expand towards the rest of the domain. 
Most methods build some form of the front boundaries explicitly.
Some methods construct the union of spheres~\cite{Li99biting:advancing,fastspherepacking}.
These methods are intractable in high dimensions because the number of intermediate-dimensional faces grows factorially with dimension. 
As a practical matter, implementing the geometric primitives for the constructions would be challenging as well.

The key innovation of \bridsonmethod~\cite{Bridson:2007:FPD} is to represent the front boundary implicitly, by a list of sample disks touching the front.
\bridsonmethod\ does rejection sampling around a prior sample,
selecting a point uniformly by volume from the $[\rconflict, \rcoverage]$ annulus around it.
The sample is removed from the front after a fixed number (30) of consecutive rejections.
Its advantage is locality, mitigating the effects of domain size. 
This enables tractable runtime in high dimensions.
\footnote{As published, step 0 constructs a background grid.
Replacing it with a $k$-d tree improves runtime from $2^{O(d)}O(n)$ to $O(d n^2),$ 
the same complexity as our \hidmethod.}

The publication is a single page sketch and does not analyze saturation by dimension.
We postulate that the method guarantees that only a small fraction of the annulus volume is unsaturated. 
However, we do not know how to bound the uncovered volume outside all annuli.
Perhaps more significantly, we have discovered that its output has an undesirable artifact, 
a sharp discontinuity in the density of points at the outer boundary of annuli; see \figref{fig:bridsonresults}.

\pargrph{Hyperplane sampling}
%
\Darts~\cite{kddarts_arxiv} uses hyperplanes for Poisson-disk sampling: select a random axis-aligned hyperplane, find its uncovered subset, and select a point from this subset. 
A rejection occurs only when the entire hyperplane is covered. 
Its advantage is that hyperplanes mitigate the effects of high dimensions.
A hyperplane is especially efficient for dealing with arrangements of spheres, because its intersection with a sphere is a lower-dimensional analytic sphere.
Its disadvantage is that it does not guarantee \emph{local} saturation, because hyperplanes are selected \emph{globally} from the entire domain.
(Global dart throwing \cite{Dippe:1985:ATS,Cook:1986:SSCG} has similar issues.)
In principle, using any dimensional hyperplane is possible, up to the dimension of the domain.
However, the difficulty is actually performing and representing the necessary geometric primitives over this object. In \Darts\ and the present work, we merely use lines, 1Dimensional hyperplanes.

Sun et al.~\shortcite{Sun:2013:LSS} samples lines and line-segments for rendering applications, including 3D motion blur, 4D lens blur, and 5D temporal light fields.
For determining sample positions it relies on subroutines that do not scale well to high dimensions.


==> all_segments_alg.tex <==
\begin{algorithm}
  \Caption{Trim all segments.}{}
  \label{alg:all_segments}
  \begin{algorithmic} [1]  
    \REQUIRE line or great circle $\linespoke$ with anchor $p$ for $\sample$
    \ENSURE all uncovered segments, of trimmed spoke $\linespokeprime$
    \STATE \COMMENT{find all intersections}
    \STATE intersections $I \leftarrow \emptyset$
    \STATE depth $\leftarrow 0$
    \FOR{each neighbor $\sampleprime$ of $\sample$}
      \STATE $\{i_+, i_-\} \leftarrow \disk(\sampleprime) \bigcap \linespoke$
      \STATE $I \leftarrow I \bigcup \{i_+, i_-\}$
      \IF{$p \in \disk(s)$}
          \STATE increment(depth)
      \ENDIF      
    \ENDFOR
    \STATE \COMMENT{find depth of intervals between intersections}
    \STATE sort($I$)
    \STATE current\_depth $\leftarrow$ depth
    \STATE interval\_start $\leftarrow$ p
    \FOR{$i \in I$}
      \IF{( $i$ is + )}
        \STATE increment(current\_depth)
        \IF{current\_depth = 1}
          \STATE $\linespokeprime \leftarrow \linespokeprime \bigcup [ \textrm{interval\_start}, i ]$
        \ENDIF
      \ENDIF
      \IF{( $i$ is - )}
        \STATE decrement(current\_depth)
        \IF{current\_depth = 0}
          \STATE interval\_start $\leftarrow i$
        \ENDIF
      \ENDIF
    \ENDFOR  
    \RETURN{} $\linespokeprime$
  \end{algorithmic}
\end{algorithm}


==> beta_by_time_fig.tex <==
\begin{figure*}[tbh]
\centering
  \subfloat[$d = 2$]
  { \label{fig:beta_time_2d}
     \includegraphics[width=0.24\linewidth]{figs/MPS_4d_new.pdf}
  }    
  \subfloat[$d = 3$]
  { \label{fig:beta_time_3d}
     \includegraphics[width=0.24\linewidth]{figs/MPS_6d_new.pdf}
  }  
  \subfloat[$d = 4$]
  { \label{fig:beta_time_4d}
     \includegraphics[width=0.24\linewidth]{figs/MPS_8d_new.pdf} 
  }
  \subfloat[$d = 5$]
  { \label{fig:beta_time_5d}
     \includegraphics[width=0.24\linewidth]{figs/MPS_10d_new.pdf} 
  }
 \Caption{Saturation $\rratio$ by time for different methods across dimension.}
 {\scott{Chonhyon running experiments to replace these figures with real ones.}}
 \label{fig:beta_by_time}
 
\end{figure*}



==> blue_noise_background.tex <==

\subsection{Definitions\nothing{ and Applications}}
\label{sec:blue_noise_background}

%\pargrph{Blue noise and saturation definitions} 
Blue noise distributions are random and well-spaced.
Randomness is characterized by the frequency spectrum of the points~\cite{Heck:2013:BNS}.
The primal data are the $d$-dimensional vectors of distances between all pairs of points, and their Fourier transform describes the spectra. 
Generally, blue noise spectra have a dark center surrounded by uniform lightness.
The Radial Distance Function (RDF) is a useful one-dimensional primal measure, and the Radial Power (RP) is its transform.
Blue noise has a step-like RP.

Well-spaced samples have two properties: samples are not too close to one another, yet are \emph{saturated} in that no domain point is too far from a sample.
We define two radii around each sample, 
$\rcoverage$ for maximum domain to sample distance, and $\rconflict$ for minimum inter-sample distance~\cite{Mitchell:2012:VRPD,Ebeida:2013:ISC}.
Their ratio $\beta = {\rcoverage}/{\rconflict}$ quantifies saturation.
There are practical random algorithms that achieve $\beta=1$  in low dimensions, but none do so in high-dimensions.
A ``relaxed MPS''~\cite{kddarts_arxiv}, where $\beta$ is bounded above by some constant larger than one, is thus a reasonable goal.
It may even be preferable for graphics applications. 
In particular, it appears to be a fundamental drawback that requiring $\rratio \le 1$ everywhere in random distributions leads to many points nearly $r$ apart. 
This RDF has an even more sharp discontinuity than a standard step function, leading to greater oscillations in the RP.

\emph{Step blue noise} has a step-like RP (mostly) free of oscillations. 
\emph{Soft blue noise} has a gradual RDF step, and both the RP \emph{and} RDF are step-like.
These are preferred because of lower aliasing in rendering applications, as demonstrated by the classical zone-plate test pattern~\cite{Heck:2013:BNS,Subr:2013:FAS:2461912.2462013}. 
Several algorithms have produced step-like blue noise, and all have done so by avoiding the requirement that $\rratio \le 1$~\cite{Heck:2013:BNS,Mitchell:2012:VRPD}.

\subsection{Applications}
%\pargrph{Blue noise applications}
Blue noise has many graphics applications, such as rendering, 
 imaging, 
 geometry,
  animation, 
  visualization, 
  and numerical computation
 \cite{Cook:1986:SSCG,Sun:2013:LSS,Chen:2013:BBN,Balzer:2009:CCPD,Fattal:2011:BNPS,deGoes:2012:BNT,Alliez:2003:APR,Oztireli:2010:SSM,Schechter:2012:GSA,Li:2010:ABNS,kddarts_arxiv}. 
%\cite{Cook:1986:SSCG,Sun:2013:LSS,Chen:2013:BBN}; 
%\cite{Balzer:2009:CCPD,Fattal:2011:BNPS,deGoes:2012:BNT}; 
%\cite{Alliez:2003:APR,Oztireli:2010:SSM}; 
%\cite{Schechter:2012:GSA};
%\cite{Li:2010:ABNS}; and
%\cite{kddarts_arxiv}. 
Randomness avoids aliasing while well-spacedness reduces noise and improves efficiency.
Saturation (but not necessarily $\rratio=1$) is important for many applications, as described in the extensive literature on MPS~\cite{Jones:2005:EGPDS,Cline:2009:DRS,Gamito:2009:AMPD,Ebeida:2011:EMP,Ebeida:2012:SAM,Yan:2013:GPA}.
We have seen an increase in the dimension of blue-noise used for rendering applications, but it is unclear how important saturation and separation are as the dimension increases. In \figref{fig:mitsuba} we demonstrate rendering using 8D sampling. 
% 6d in prior papers

% why
\pargrph{Global optimization}
%
Optimization is useful for many traditional graphics applications: 
optimal light source placement~\cite{Gumhold:2002:MEL:602099.602141}, object and camera trajectories, object reflectance, etc.
The optimization problem is often high-dimensional even when the underlying graphics quantity is low dimensional: there is one dimension for every parameter describing the solution. For example, the configuration space of placing $k$ light sources in a 3D domain is $3k$ dimensional.
Soft shadows are generated by placing point-sources at blue-noise locations sampled from an area light source~\cite{nvidia:softshadows}.
Finding the optimal positions to minimize the number of lights needed to extract all depth discontinuities from shadows %in a scene 
using a multiflash camera is a high-dimensional  optimization problem that is currently solved approximately~\cite{VaqueroCVPR2008}.  
%

Many applications require global optimization, because there are local minima that are much less desirable than the global minimum.
Since following local gradients leads to getting stuck in these minima, many black-box global optimization algorithms make use of sampling.
Generating well-spaced samples becomes more critical for efficiency as the parameter space increases in dimension.

\pargrph{Motion planning}
Robotic optimal path planning is a specialized form of global optimization that exploits the problem structure.  Some robot configurations are inadmissible because they imply a collision with the environment or a self-collision.
The space of robot configurations is vast, one dimension for each degree of freedom of the robot.
Increasing the complexity and realism of robots and environments increases the dimension of the problem.
It is intractable to construct the boundary between admissible and inadmissible configurations, so most algorithms rely on marching from one admissible configuration point to a nearby one, and checking that it, too, is admissible. Checking a point is expensive.
It is most efficient to explore these paths in parallel, yet one must avoid wasting time by parallel threads exploring nearly identical paths.
As such, we precomputed a blue noise sampling of configurations, and restrict threads to only consider those points (and predetermined local refinements), so they can tell if another thread has already considered it.
Our prior work \cite{Park:2013:RT} was limited to 6 dimensions, because we were unable to produce blue noise in higher dimensions. 
In this paper we produce blue noise in 23 dimensions and demonstrate planning over it.


==> bridson_experiment.tex <==

\subsection{Comparison to \bridsonmethod}
\label{sec:bridsonexperiments}
Bridson \shortcite{Bridson:2007:FPD} has shared the code for \bridsonmethod\, which produces aperiodic samples.
We also re-implemented the method as \bridsonmethodours\ in our framework, to support periodic domains.
For both implementations, the main shortcoming we observe is a discontinuity in the RDF distribution at the outer annulus radius, $2r$; see \Cref{fig:bridsonrdf2d}.
The discontinuity is severe for $d=2$, and lessens as the dimension increases.
Additional results may be found in \Cref{fig:bridsonextra} in \Cref{sec:bridsonappendix}.
The number of sample attempts is fixed at 30 regardless of dimension.
Our method for obtaining provable bounds on $\rratio$ for \hidmethod\ does not carry through for point samples from an annulus.
In practice, we observe that \bridsonmethodours\ in $d$ dimensions produces median $\rratio$ values similar to \linespokesalg\ in $d+1$ dimensions. Intuitively, spoke sampling instead of point sampling effectively reduces the dimension by one.
%This follows using the same analysis technique we use for our method, and noting that 
%the volume ratio between the annulus and the disk it surrounds is $2^\dimnumber - 1.$
%Worse, we know of no bound on the uncovered gap volume (or its radius) \emph{outside all annuli.}
%

% Bridson table of results
% using the outlier beta is not a stable indicator
%\begin{table}[!ht]
%\centering
%\tabtextsize
%\begin{threeparttable}[b]
%% caption can't go here
%\begin{tabular}{rrrr}
%% caption can't go here
%\toprule
%$\dimnumber$ & $\rratio$ & $\samplenumber$ & $r$ \\ 
%\midrule
%2 & 1.25   & 154,167  & 0.002\\
%3 & 1.36   & 143,633  & 0.016\\
%4 & 1.38  & 48,075   & 0.06\\
%5 & 1.63 &  69,991   & 0.1\\
%\bottomrule
%% \hspace{0.4\columnwidth}
%\end{tabular}
%% \vspace{-12pt}
%\end{threeparttable}
%\Caption{\bridsonmethod\ experimental results.}
%{} 
%\label{tab:bridsonbeta}
%\end{table}


\begin{figure}[tbh]
	\centering
	\subfloat[RDF]
	{
		\label{fig:bridsonrdf2d}
		\includegraphics[height=1.2in]{figs/bridsonexperiments/2d/RDFhistogram.png}
	}
	\subfloat[spectrum]
	{
		\label{fig:bridsonfft}
		\includegraphics[height=1.2in]{figs/bridsonexperiments/2d/fftslice.png}
	}
	\caption{\bridsonmethod\ results in $d=2$.}
	\label{fig:bridsonresults}
\end{figure}



==> building_blocks.tex <==
\subsection{Combining Advancing Front and Hyperplanes}
\label{sec:building_blocks}

%Despite the desirability of sampling in high dimensions, most capabilities are low dimensional, in part because of the curse of dimensionality --- many blue noise algorithms do not scale well to high dimensions, especially when seeking high saturation.

The sampling methods that scale well with dimension do not provide a guarantee of local saturation. 
Those providing local saturation have exponential complexity.
The algorithms closest to obtaining both of these goals are based on
advancing-front~\cite{firstspheremesh,Bridson:2007:FPD} or \kddarts~\cite{kddarts_arxiv}.


\pargrph{\Hidmethod}
Our key idea is to combine the advantages of these two.
%the local saturation of \bridsonmethod\ and the dimension-mitigation of \kddarts.
Specifically, \hidmethod\ replaces the point-sampling of \bridsonmethod\ with hyperplane sampling. 
Conceptually, a \emph{spoke} is a $k$-dimensional hyperplane passing through a point, at a random orientation.
In practice we use 1D lines.
See \figref{fig:spokes}.

\input{spokes_new_fig}

We still use only a constant number (12) of consecutive rejections before advancing the front, retaining good run-time scalability across dimensions. However, spokes provide a local saturation distance guarantee that is the \emph{same in all dimensions}. 
They also enable \emph{step} blue noise. Selecting a sample point uniformly from a segment results in traditional blue noise.
We achieve step blue noise by selecting the sample point non-uniformly from a spoke.
We achieve  \emph{soft step blue noise} by generating a second spoke through the first-spoke point, and selecting the final sample from it.  
These two spokes mimic the two radii in Mitchell et al.~\shortcite{Mitchell:2012:VRPD}.





==> common/ascr_sandia_acknowledgement.tex <==
% \small
% include this if ASCR funding WAS used
This material is based upon work supported by the U.S. Department of Energy, Office of Science, Office of Advanced Scientific Computing Research (ASCR), Applied Mathematics Program. 
% always include this
Sandia National Laboratories is a multi-program laboratory managed and operated by Sandia Corporation, a wholly owned subsidiary of Lockheed Martin Corporation, for the U.S. Department of Energy's National Nuclear Security Administration under contract DE-AC04-94AL85000. 


==> common/linenofix.tex <==
%http://phaseportrait.blogspot.com/2007/08/lineno-and-amsmath-compatibility.html
%Fix for corruption between amsmath and lineno
\newcommand*\patchAmsMathEnvironmentForLineno[1]{%
  \expandafter\let\csname old#1\expandafter\endcsname\csname #1\endcsname
  \expandafter\let\csname oldend#1\expandafter\endcsname\csname end#1\endcsname
  \renewenvironment{#1}%
     {\linenomath\csname old#1\endcsname}%
     {\csname oldend#1\endcsname\endlinenomath}}%
\newcommand*\patchBothAmsMathEnvironmentsForLineno[1]{%
  \patchAmsMathEnvironmentForLineno{#1}%
  \patchAmsMathEnvironmentForLineno{#1*}}%
\AtBeginDocument{%
\patchBothAmsMathEnvironmentsForLineno{equation}%
\patchBothAmsMathEnvironmentsForLineno{align}%
\patchBothAmsMathEnvironmentsForLineno{flalign}%
\patchBothAmsMathEnvironmentsForLineno{alignat}%
\patchBothAmsMathEnvironmentsForLineno{gather}%
\patchBothAmsMathEnvironmentsForLineno{multline}%
}


==> common/macros.tex <==
\input{../common/macroscommon}
\newtheorem{theorem}{Theorem}[section]
\newtheorem{proposition}[theorem]{Proposition}

==> common/package.tex <==

\usepackage{times,color}
\usepackage{parskip}
%\usepackage{epsfig}
%\usepackage{psfig}
%\usepackage[pdftex]{graphicx} % new acmsiggraph.cls
\usepackage{ifthen}
%\usepackage[draft]{hyperref} % new acmsiggraph.cls
\usepackage{float}
\usepackage{alltt}

\usepackage{amssymb}
\usepackage{mathenv}
\usepackage{amsmath}
\usepackage{array}
\usepackage{amsthm}


%\usepackage{rotating}
\usepackage{newlfont} % for Box
%\usepackage{ulem}
\usepackage{floatflt}
\usepackage{wrapfig}
\usepackage{fixltx2e}
\usepackage{subfig} % for subfloat
\usepackage{multirow}
\usepackage{wasysym}
\usepackage{booktabs} %for toprule, midrule, bottomrule in table
\usepackage{slashbox} %for toprule, midrule, bottomrule in table
\usepackage{mwe}

\usepackage{threeparttable}

\usepackage{cleveref}

%% pseudocode
\usepackage{savesym}
\savesymbol{AND}

\usepackage{algorithm}
%\usepackage{algorithmic}

%
% algcompatible defines algorithmic, conflict with above algorithmic package
\usepackage[noend]{algcompatible}
%
%

%\savesymbol{algorithmicincident}
%\usepackage{algorithmic}
%\usepackage{algcompatible}
%\usepackage{algorithm}
%\usepackage{algorithmic}
%\usepackage{algorithmicx}
%\usepackage{algpseudocode}
%\usepackage{xspace}

\usepackage{hyperref}
\hypersetup{
    colorlinks,%
    citecolor=black,%
    filecolor=black,%
    linkcolor=black,%
    urlcolor=black
}


==> contribution.tex <==
\subsection{Contribution}
The contribution of this paper can be summarized as follows:
\begin{itemize}
\item
The idea of \emph{\hidmethod,} which combines the advantages of the locality of advancing-front 
%(\bridsonmethod) 
with the dimension-mitigation of hyperplane sampling;
% (\kddarts);

\item
Direct algorithms for traditional, step, and smooth blue noise;

\item
Algorithms that scale to high dimensions;

\item
Proven and demonstrated time, memory and saturation bounds;

%\item
%Output that is locally saturated and well spaced: the distance between any two samples is at least $r$, and with high probability the distance between any domain point and its nearest sample is at most $2r$ for \linespokesalg; 

\item
Open source software for our algorithms~\cite{spokedartspubliccode};

\item
Applications using spokes for high dimensional Delaunay graphs, global optimization, and motion planning.
\end{itemize}


To our knowledge, we provide the first feasible method to produce probabilistically-guaranteed locally-saturated blue noise in high dimensions,
and the first direct methods for step and soft blue noise 
in $d>2$.
% TwoRadii MPS from "Variable Radius..." paper did 2d



==> discussion.tex <==

\section{Discussion}
\label{sec:stepbluenoise}

Here we discuss the algorithmic choices described for blue noise and step blue noise

==> experiements.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\section{Experimental Results}
\label{sec:exp}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

In this section, we demonstrate the capabilities of our algorithm through a number of practical experiements. Note that SpokeDartsPublic software is available as open source~\cite{spokedartspubliccode}, and may be used to verify the experimental results.

\subsection{Blue Noise by Dimension and Method}

\Cref{fig:rdf_spectra_teaser} shows the blue noise characteristics of our algorithm (and its variations in Appendix~\ref{sec:alg_variants}), for 2D periodic domains.
Their spectra do not vary significantly as the dimension increases.
See \Cref{fig:rdf_spectra_ld,fig:rdf_spectra_fd,fig:rdftwo} in \Cref{sec:additional_results} for spectra examples in $\dimnumber=3, 4, 5$.
\Cref{fig:rdf} shows the Radial Distance Function (RDF) for $\dimnumber=6$.
For coarse samplings of aperiodic domains, the boundary significantly affects the distribution characteristics.

\input{rdf_fig}
\input{coverage_fig}
\input{betamedian_fig}
\input{rdf_spectra_teaser_fig}
% no point in showing more until we can go beyond d=6 for periodic domains

%\input{rdf_spectra_fig} - in appendix

The RDF and spectra of line- and two-spokes differ significantly. However, they have similar $\rratio$ distributions, after scaling by $\rratio_{two} \approx 2 \rratio_{line}$, as described in the next section.


% samitch: moved from the analysis section. OK to clean up, move to appendix, or whatever
\Cref{fig:local_beta} shows the distribution of $\rcoverage$ for $\hammerlimit=12$.
\Cref{fig:coverage_ext} shows how increasing $\hammerlimit$ affects the output saturation.
%\Cref{fig:coverage} shows \linespokesalg's achieved and guaranteed $\rratio$ for $\dimnumber=4$ as $\hammerlimit$ increases. 
As the dimension increases the distributions tend to resemble a Gaussian and become more sharply peaked.
While the theory guarantees are invariant in dimension, in practice \linespokesalg\ and \twospokesalg\ produce slightly larger $\rratio$ in higher dimensions.
\Cref{fig:betamedian} shows the median $\rratio$ by method and dimension.

\begin{itemize}
	\item \Linespokesalg\ has $\rratio^*=2$ and median $\rratio \approx $ 0.9--1.2 as $d=$ 2--5.
	\item \Twospokesalg\ has $\rratio^*=4$ and median $\rratio \approx $ 1.8--2.4 as $d=$ 2--5.
	\item \Favoredspokesalg\ has median $\rratio \approx 1.5$ regardless of $d$.
\end{itemize}

%See \Cref{fig:local_beta_extra} in \Cref{sec:additional_results} for more details.
Although we can create blue noise distributions in high dimensions, our ability to analyze their $\rratio$ is limited by the challenge of computing Voronoi vertices. We use QHull, and for large $\dimnumber$ and reasonable $\samplenumber,$ QHull runs out of memory (and time).



==> gopt_alg.tex <==

% scott

\begin{algorithm}
  \begin{algorithmic}[1]
    
    \REQUIRE target function $f$ over domain $\domainsym$
    \ENSURE minimum $f^\ast$ found

    \STATE $s = \funct{Center}(\domainsym)$ \pcomment{any sample point}
    \STATE $\sampleset = \{s\}$ \pcomment{sample set}
    \STATE $\fset \leftarrow \{ f(\sample) \}$ \pcomment{function values at samples}
    \STATE $f^\ast \leftarrow f(\sample)$ \pcomment{minimum value found so far}
    \STATE $\dset = \{ |\domainsym|\}$ \pcomment{set of cell size estimates} %, $\{d_i\}$}

    \WHILE{computational budget is not exhausted}

      \STATE $\lowercellset =  \funct{LowerHull}(\fset, \dset, f^\ast)$
      \STATE $\sample \leftarrow \funct{RandomSelect}(\lowercellset)$
      \STATE $ r \leftarrow \funct{inradius}(\dgraph^\ast(\sample))$ \pcomment{nearest-neighbor / 2}
      \STATE $\spoke \leftarrow \funct{RandomSpoke}(\sample, r, [ r, \infty] )$
      \STATE $\spoke \leftarrow \funct{TrimSpoke}(\spoke, r, \funct{hyperplanes}(\dgraph^\ast(\sample))$ %\pcomment{see \Cref{alg:spoke}}
      \STATE $\sampleprime \leftarrow \funct{RandomSample}(\spoke)$
      \STATE $\sampleset \leftarrow  \sampleset \bigcup \{\sampleprime\}$
      \STATE $\fset \leftarrow  \fset \bigcup \{f(\sampleprime)\}$
      \STATE $f^\ast \leftarrow \funct{min}(f^\ast,f(\sampleprime))$
    
      % update graph
      \STATE $(\dgraph^\ast, \dset) \leftarrow \funct{DelaunayAdd}(\dgraph^\ast, \sampleprime)$ \pcomment{\Cref{alg:meshing}}

    \ENDWHILE
    \RETURN{} $f^\ast$
  \end{algorithmic}
  \Caption{Opt-darts global Lipschitzian optimization.}{}
  \label{alg:gopt}
\end{algorithm}


% old version of the algorithm
\nothing{
\begin{algorithm}
  \begin{algorithmic}[1]
    
    \REQUIRE target function $f$ over domain $\domainsym$
    \ENSURE global minimum $f^\ast$

    \STATE $f^\ast \leftarrow \infty$
    \STATE $\dgraph^\ast \leftarrow \domainsym$ \pcomment{Delaunay graph}
    \STATE $\sampleset \leftarrow \emptyset$ \pcomment{sample set, initially empty}
    \WHILE{$\cellset \leftarrow \funct{PotentialCells}(f,f^\ast,\dgraph^\ast)$ not empty}  
    \STATE \pcomment{condition in \Cref{eqn:direct_condition_1} and \Cref{eqn:direct_condition_2}}
    \WHILE{$\cellset$ not empty}  
    \STATE $\cell \leftarrow \funct{RandomSelectAndRemove}(\cellset)$
    \STATE $\sample \leftarrow \funct{OneSpokeSample}(\cell)$ \pcomment{see \Cref{alg:spoke}}
    \STATE $f^\ast \leftarrow \funct{min}(f^\ast,f(\sample))$
    \STATE $\sampleset \leftarrow \sampleset \bigcup \left\{ \sample \right\}$
    \STATE $\dgraph^\ast \leftarrow \funct{DelaunayAdd}(\nothing{\domainsym,} \dgraph^\ast, \sample)$ \pcomment{\Cref{alg:meshing}}
    \ENDWHILE
    \ENDWHILE
    \RETURN{} $f^\ast$
  \end{algorithmic}
  \Caption{Opt-darts global Lipschitzian optimization.}
{For clarity, we assume looking for global minimum as in \Cref{eqn:direct_condition_1} and \Cref{eqn:direct_condition_2}.
\mohamed{I am not sure what is this algorithm for?!. Opt-dart: For each sample we need to have an estimate of $h_i$: the distance between it and its furthest Vornoi cell \liyi{This is what \Cref{eqn:direct_condition_1} is for}. \liyi{OneSpokeSample is for what you described below.} We throw spokes for this purpose and trim them using the boundaries of that Voronoi cell. the maximum length of the trimmed spokes is our estimate for $h_i$. When we insert a new sample point inside a candidate cell we sample point inside that Voronoi cell using the same approach with additional constraint: the points has to be outside the inscribed circle of that Voronoi cell. }
\liyi{Please see my answer above. If you find anything needing improvement, update the code and the main text directly. I cannot be your interpreter all the time. A key thing about presentation is modularity: each one of our application should build upon cleanly on our core algorithms, e.g. using just OneSpokeSample. It is not OK to have to repeat the basic algorithm again in a slight variation. It is not clean algorithm design or thinking, and poor presentation reflects that.}
}
  %\label{alg:gopt}
\end{algorithm}
}%nothing


==> gopt_demo_convexhull_fig.tex <==
\begin{figure}[tbh] 
 \centering
 \subfloat[Iteration 0 (n = 0)]
   {
     \includegraphics[width=0.22\linewidth]{figs/DIRECT_convex_hull_1.pdf} $\,$
     \includegraphics[width=0.22\linewidth]{figs/opt_darts_convex_hull_1.pdf}
 }
  \subfloat[iteration 1 (n = 3, 2)]
   {
     \includegraphics[width=0.22\linewidth]{figs/DIRECT_convex_hull_3.pdf} $\,$
     \includegraphics[width=0.22\linewidth]{figs/opt_darts_convex_hull_2.pdf}
   }
 
  \subfloat[iteration 2 (n = 5, 3)]
   {
     \includegraphics[width=0.22\linewidth]{figs/DIRECT_convex_hull_5.pdf} $\,$
     \includegraphics[width=0.22\linewidth]{figs/opt_darts_convex_hull_3.pdf}
   }
  \subfloat[iteration 3 (n = 7, 4)]
  {
     \includegraphics[width=0.22\linewidth]{figs/DIRECT_convex_hull_7.pdf} $\,$
     \includegraphics[width=0.22\linewidth]{figs/opt_darts_convex_hull_4.pdf}
  } 
 
  \subfloat[n = 31]
   {
     \includegraphics[width=0.22\linewidth]{figs/DIRECT_convex_hull_31.pdf} $\,$
     \includegraphics[width=0.22\linewidth]{figs/opt_darts_convex_hull_31.pdf}
   }
  \subfloat[n = 101]
  {
     \includegraphics[width=0.22\linewidth]{figs/DIRECT_convex_hull_101.pdf} $\,$
     \includegraphics[width=0.22\linewidth]{figs/opt_darts_convex_hull_101.pdf}
  } 
  
  \subfloat[n = 301]
  {
     \includegraphics[width=0.22\linewidth]{figs/DIRECT_convex_hull_301.pdf} $\,$
     \includegraphics[width=0.22\linewidth]{figs/opt_darts_convex_hull_301.pdf}
  } 
\subfloat[n = 601]
  {
     \includegraphics[width=0.22\linewidth]{figs/DIRECT_convex_hull_601.pdf} $\,$
     \includegraphics[width=0.22\linewidth]{figs/opt_darts_convex_hull_601.pdf}
  } 
 
  \Caption{Evolution of convex hull of DIRECT (left) and our DIVOR method (right) while exploring the function in \Cref{fig:gopt_demo_fspace}.}
  {}
    \label{fig:gopt_demo_convexhull}
\end{figure}  


==> gopt_demo_fspace_fig.tex <==
% we don't use ``nodes'' we use ``cells'' or ``samples''
\begin{figure}[tbh] 
 \centering
 \subfloat[iteration 0, \# samples (1,1)]
   {
     \includegraphics[width=0.22\linewidth]{figs/DIRECT_1.pdf} $\,$
     \includegraphics[width=0.22\linewidth]{figs/opt_darts_1.pdf}
 }
  \subfloat[iteration 1, \# samples (3, 2)]
   {
     \includegraphics[width=0.22\linewidth]{figs/DIRECT_3.pdf} $\,$
     \includegraphics[width=0.22\linewidth]{figs/opt_darts_2.pdf}
   }
 
  \subfloat[iteration 2, \# samples (5, 3)]
   {
     \includegraphics[width=0.22\linewidth]{figs/DIRECT_5.pdf} $\,$
     \includegraphics[width=0.22\linewidth]{figs/opt_darts_3.pdf}
   }
  \subfloat[iteration 3, \# samples (7, 4)]
  {
     \includegraphics[width=0.22\linewidth]{figs/DIRECT_7.pdf} $\,$
     \includegraphics[width=0.22\linewidth]{figs/opt_darts_4.pdf}
  } 
 
  \subfloat[\# samples (31, 31)]
   {
     \includegraphics[width=0.22\linewidth]{figs/DIRECT_31.pdf} $\,$
     \includegraphics[width=0.22\linewidth]{figs/opt_darts_31.pdf}
   }
  \subfloat[\# samples (101, 101)]
  {
     \includegraphics[width=0.22\linewidth]{figs/DIRECT_101.pdf} $\,$
     \includegraphics[width=0.22\linewidth]{figs/opt_darts_101.pdf}
  } 
  
  \subfloat[\# samples (301, 301)]
  {
     \includegraphics[width=0.22\linewidth]{figs/DIRECT_301.pdf} $\,$
     \includegraphics[width=0.22\linewidth]{figs/opt_darts_301.pdf}
  } 
\subfloat[\# samples (601, 601)]
  {
     \includegraphics[width=0.22\linewidth]{figs/DIRECT_601.pdf} $\,$
     \includegraphics[width=0.22\linewidth]{figs/opt_darts_601.pdf}
  } 

\subfloat[\# samples (999, 999)]
  {
     \includegraphics[width=0.22\linewidth]{figs/DIRECT_999.pdf} $\,$
     \includegraphics[width=0.22\linewidth]{figs/opt_darts_999.pdf}
  } 
  \subfloat[Smooth Herbie\nothing{ \mohamed{function driving sampling in the rest of the figures here}}]
  {\label{fig:gopt_demo_fspace_smooth_herbie}
   \hspace{0.10\linewidth}
   \includegraphics[width=0.24\linewidth]{figs/HerbieSmooth.pdf}
   \hspace{0.10\linewidth}
  } 
 
  \Caption{Comparing DIRECT (left) and our Opt-darts method (right) while exploring the smooth Herbie function \protect\subref{fig:gopt_demo_fspace_smooth_herbie}.}
  {%
    We list the number of samples used by each as (DIRECT, Opt-darts).
  }
    \label{fig:gopt_demo_fspace}
\end{figure}

\nothing{
\liyi{(January 21, 2014) it is not clear to me in this didactic example how and why our method is better than DIRECT.}
}%nothing

\nothing{
 \subfloat[Herbie \mohamed{We may take this our if you like}]
  {
     \includegraphics[width=0.23\linewidth]{figs/Herbie.pdf}
     \label{fig:gopt_demo_fspace_herbie}
  } 

\liyi{(January 14, 2014) What are \subref{fig:gopt_demo_fspace_smooth_herbie} and \subref{fig:gopt_demo_fspace_herbie} for? Are they different functions or visualization obtained by DIRECT and our method, respectively? (The former doesn't make sense while the latter needs more explanation.)} \mohamed{These are two close function (with the same trend) one is smooth and the other one has oscillating behavior. In our experiments we will have results for Herbie and results for Smooth Herbie so I wanted t use the space to give an idea to the reader of how they look like. Smooth Herbie is crucial here cause one can relate the density of the points in the demo and where the humps of the function occur.}
\liyi{OK to avoid confusion let's just leave smooth Herbie here.}
}%nothing


==> gopt_demo_fspace_fig_body.tex <==
\begin{figure}[!b] 
 \centering
    \setlength{\tabcolsep}{3pt}
    \resizebox{\columnwidth}{!}{
		\begin{tabular}{cccc}
			\rotatebox[origin=l]{90}{DIRECT}
			\includegraphics[height=1in]{figs/DIRECT_7.pdf}
			\includegraphics[height=1in]{figs/DIRECT_31.pdf}
			\includegraphics[height=1in]{figs/DIRECT_101.pdf}
			\\
			\rotatebox[origin=l]{90}{Opt-darts}
			\includegraphics[height=1in]{figs/opt_darts_4.pdf}
			\includegraphics[height=1in]{figs/opt_darts_31.pdf}
			\includegraphics[height=1in]{figs/opt_darts_101.pdf}
%  \subfloat[Smooth Herbie]
%  {\label{fig:gopt_demo_fspace_smooth_herbie}
%   \hspace{0.10\linewidth}
%   \multicolumn{2}{c}{\includegraphics[height=1in]{figs/HerbieSmooth.pdf}} \\
%   \multicolumn{2}{c}{\tiny{smooth Herbie function}}
%   \hspace{0.10\linewidth}
%  } 
 		\end{tabular}
}
  \Caption{DIRECT (top) vs.\ Opt-darts (bottom) for discovering the global maximum of the didactic ``Smooth Herbie'' function.}
  {Opt-darts more efficiently places samples. Opt-darts cells are better-shaped, leading to a better choice of which cells to refine. This concentrates samples nearer to the true optimum, leading to faster convergence, about a 4x speedup in practice.}
    \label{fig:gopt_demo_fspace_body}
\end{figure}


==> gopt_main_fig.tex <==
\begin{figure}[tb] 
 \centering
   \subfloat[rectangular cells]
   {
     \label{fig:bad_rect}
     \includegraphics[width=0.45\linewidth]{figs/bad_rect.pdf}
  }
  \subfloat[Voronoi cells]
   {
     \label{fig:good_vor}
     \includegraphics[width=0.4555\linewidth]{figs/bad_rect_vor.pdf}
  }
  \Caption{Main weakness of DIRECT \protect\cite{jones1993lipschitzian}.}
  {Rectangular partitions \subref{fig:bad_rect} can give misleading estimates of sample-neighborhood sizes. 
Voronoi cell partitions \subref{fig:good_vor} improve these estimates, especially for high dimensions.
For example, the size of the relevant neighborhood of point A in \subref{fig:bad_rect} is overestimated, 
since all its corners are actually closer to other sample points, e.g.\ 
$p$ is closer to D, as seen in \subref{fig:good_vor}.
  }
    \label{fig:gopt_main}
\end{figure}  

\nothing{\liyi{(January 19, 2014) We don't mention known $K$.}

  \subfloat[\nothing{discarded subregions (rectangles vs balls)}]
  {
    \label{fig:gopt_discarded}
      \includegraphics[width=0.3\linewidth]{figs/bad_rect_2.pdf}
   }

The volume of discarded disjoint rectangle is always less than the volume of the union of the overlapping disks that contains these rectangles \subref{fig:gopt_discarded}.
\liyi{(January 13, 2014) part \subref{fig:gopt_discarded} is not clear to me.} \mohamed{I was simply trying to make the argument that the volume of some disjoint recatngles (discarded regions in DIRECT) is always less than the volume of their covering spheres (Discraded regions in Opt-darts) even if those spheres overlapp. In that sense opt-dart should be always faster than DIRECT. }
\liyi{(January 14, 2014) This is confusing. I thought our algorithm is keeping track of Voronoi cells instead of rectangular cells as in DIRECT, right? If so, I assume we decide whether to pursue a cell entirely, otherwise the tracking algorithm can be quite complex. If so I cannot see how the sphere thing comes into play. Overall, if \subref{fig:gopt_discarded} is indeed a major point, it should be spelled out in the main text. It is not right now.}
\mohamed{Sorry for confusing you again. This figure is to emphasize that spheres are better to discard regions (if K is known) than rectangles. If K is known the discard region in opt-darts is green and the discarder regions in DIRECT is red which is much less than the green. I hope it is clear now.}
}%nothing


==> gopt_performance_tab.tex <==
\begin{table}
  \centering
  \tabtextsize
  \resizebox{\columnwidth}{!}{%
    %\renewcommand{\arraystretch}{1.2}
    \begin{tabular}{|c| r| r| r|r|}
      \hline
      Benchmark       & dimension      & DIRECT         & Opt-darts  & Speedup\\
      \hline
      Easom		                  &	6 	&	4987 	&	1912 	& 2.60$\times$	\\					
      Easom	                           &	 8 	&	64405	&	8480  	& 7.59$\times$	\\			
      Easom                           &	10	&	816937	&	19081 	& 	42.81$\times$ \\	
      Bohachevsky               & 	7	&	 10315	         & 	 2125	         &  4.85  $\times$ \\
      Exponential               & 	10	&	 13481	         & 	 7807	         &  1.72  $\times$ \\
      Exponential               & 	15	&	36890 	         & 	 10316	         &    3.57$\times$ \\
      \hline			
      
    \end{tabular}%
  }
 % relative error $\epsilon = \dfrac{f^\ast - f_{min}}{f_{max} - f_{min}} = 10^{-4}$.}
\Caption{Performance comparison of DIRECT and our Opt-darts method, measured by the number of function evaluations needed to find the global minimum within $10^{-4}$ relative error.}
{Since our method is random, results are the averages over 100 runs.
\liyi{Please describe these functions a bit and explain why we choose them.}
}
\label{tab:gopt_performance}
\end{table}

\nothing{
\liyi{(January 30, 2014) I just realized a major issue here: we need to report wall clock time, not just number of function evaluations. In particular, I presume it is cheaper to construct DIRECT's rectangular cells than our Voronoi cells.}
\mohamed{
This is not an issue at all. We are assuming that function evaluations are not cheap (e.g. each one may take one minute or more which is typical in most applications. Count of function evaluations becomes more significant and is a standard thing to report. We are indeed slower than DIRECT with regard to clock time. However the total time consumed should not be an issue as long as the function evaluation is more expensive than both algorithms. )
}%mohamed
\liyi{(February 3, 2014)
OK I hope the reviewers will buy this in our rebuttal (I won't be surprised at all to see this as a review question).
}%liyi
}%nothing

\nothing{
\mohamed{Not true yet, I am using fewer experiments than that: Due to the random nature of our method, each result is averaged from 100 different runs.}
\liyi{spell out the target error, like percentage?}
\mohamed{done. $\epsilon = \dfrac{f_{best} - f_{min}}{f_{max} - f_{min}}$}

}%nothing


==> hackbibstyle.tex <==
\setlength{\topsep}{0ex}
\setlength{\itemsep}{0ex}
\setlength{\partopsep}{0ex}
\setlength{\parsep}{0ex}
\setlength{\parskip}{1ex} %1.0ex original
%\footnotesize %\liyi{this won't pass Stephen Spencer's muster}


==> line_spoke_alg.tex <==
\begin{algorithm}
  \Caption{TrimAnchor.}{}
  \label{alg:anchored_point}
  \begin{algorithmic} [1]
    \REQUIRE anchor $\anchor$ of spoke for sample $\sample$
    \ENSURE uncovered $\anchor$ or empty
    \FOR{each neighbor $\sampleprime \in \neighbors(\sample)$}
      \IF{$\| a - \sampleprime \|^2 < r^2$}
         \RETURN{} empty %$\linespokeprime$
       \ENDIF
     \ENDFOR       
     \RETURN{} $\anchor$
  \end{algorithmic}
\end{algorithm}


\begin{algorithm}
  \Caption{TrimInterval.}{}
  \label{alg:anchored_segment}
  \begin{algorithmic} [1]
    \REQUIRE spoke $\linespoke$ with interval $\interval$, anchored at $\anchor$
    \ENSURE  trimmed $\linespoke$ with uncovered interval containing $\anchor$
    \FOR{each neighbor $\sampleprime \in \neighbors(\sample)$}
    \STATE $\interval(\linespoke) \leftarrow \interval(\linespoke) -  \funct{Disk}(\sampleprime)$
    \STATE $\interval(\linespoke) \leftarrow$ segment of $\linespoke$ containing $\anchor$, if any
%    \IF{$\linespokeprime$ is empty}
%    \RETURN{} empty %$\linespokeprime$
%    \ENDIF
    \ENDFOR
    \RETURN{} $\linespoke$
  \end{algorithmic}
\end{algorithm}


==> local_beta_fig.tex <==

\begin{figure}[tbh]
  \centering
  %2d
%   {{$\dimnumber=2$,  $\samplenumber \approx$ 110,000.}} \hspace{0.5in}
%   {{$\dimnumber=4$, $\samplenumber \approx$  70,000.}}
   {\hspace{11pt} {$\dimnumber=2$}} \hspace{1.28in}
   {{$\dimnumber=4$}}
   
%   {\rotatebox{90}{$\dimnumber=4$, $\samplenumber \approx$  70,000.}}
%2d

{\rotatebox{90}{\hspace{20pt} \Linespokesalg}}
%   \subfloat[\Linespokesalg]
   {
       \includegraphics[width=0.46\linewidth]{figs/beta_farthestvoronoi/2d/VoronoiHistogram_spoke_beta.png}
    }    
%4d
%   \subfloat[\Linespokesalg]
   {
       \includegraphics[width=0.46\linewidth]{figs/beta_farthestvoronoi/4d/VoronoiHistogram_spoke_beta.png}
    }

{\rotatebox{90}{\hspace{15pt} \Favoredspokesalg}}
%2d
%   \subfloat[\Favoredspokesalg]
   {
       \includegraphics[width=0.46\linewidth]{figs/beta_farthestvoronoi/2d/VoronoiHistogram_favored_beta.png}
    }
%4d
%   \subfloat[\Favoredspokesalg]
   {
       \includegraphics[width=0.46\linewidth]{figs/beta_farthestvoronoi/4d/VoronoiHistogram_favored_beta.png}
    }
    
    {\rotatebox{90}{\hspace{22pt} \Twospokesalg}}
    %2d
%   \subfloat[\Twospokesalg]
   {
       \includegraphics[width=0.46\linewidth]{figs/beta_farthestvoronoi/2d/VoronoiHistogram_two_beta.png}
    }
    %4d
%   \subfloat[\Twospokesalg]
   {
       \includegraphics[width=0.46\linewidth]{figs/beta_farthestvoronoi/4d/VoronoiHistogram_two_beta.png}
    }
    


   \Caption{%
$\rratio$ histograms by method.}
{%
Data are the distances from each sample to its farthest Voronoi vertex.
\liyi{(June 23, 2016) All plots should share the same horizontal and vertical axis scaling as otherwise the juxtaposition is very confusing and misleading.}%
   }
  \label{fig:local_beta}
\end{figure}


==> m_b_d_fig.tex <==
% m_b_d_fig.tex
\begin{figure}[tbh]
  \centering

   \subfloat[full scale]
   {
    \label{fig:m_b_d_full}
    \includegraphics[width=0.48\linewidth]{figs/m_b_d.pdf}
   }    
   \subfloat[zoom in]
   {
    \label{fig:m_b_d_zoom}
     \includegraphics[width=0.48\linewidth]{figs/m_b_d_zoom.pdf}
   }
  \Caption{Illustration of \Cref{eq:m_in_n_body} with $\epsilon = 10^{-5}.$}
 {Only 12 successive misses per sample are required to achieve $\rratio=2$, regardless of $\dimnumber$.}
 \label{fig:m_b_d}
 
\end{figure}



==> m_div_n_body_tab.tex <==
% three part table
%\setlength{\tabcolsep}{12pt}
\begin{table}[!ht]
\centering
\tabtextsize
\begin{threeparttable}[b]
% caption can't go here
\begin{tabular}{r|rrrr}
% caption can't go here
\toprule
\backslashbox{d}{$\rratio$} & $2$ & $1.5$ & $1.25$ & $1.125$ \\
%$d$ & $\beta=2$ & $\beta=1.5$ & $\beta=1.25$ & $\beta=1.125$ \\
%       & $x=1/4$ & $x=1/9$ & $x=1/25$ & $x=1/81$ \\
\midrule
2   & 12 & 24 & 47 & 93\\
3   & 12 & 47 & 185 & 737\\
4   & 12 & 93 & 737 &  5900 \\
5   & 12 & 185 & 3.0e3 & 4.8e4 \\
6   & 12 & 369 & 1.2e4 &  3.8e5 \\
7   & 12 & 737 & 4.8e4 & 3.1e6 \\
8   & 12 & 1.5e3 & 1.9e5 & 2.5e7 \\
9   & 12 & 3.0e3 & 7.6e5 & 2.0e8 \\
10 & 12 & 5.9e3 & 3.1e6 & 1.6e9 \\
20 & 12 & 6.1e6 & 3.2e12 & 1.7e18 \\
30 & 12 & 6.2e9 & 3.4e18 & 1.8e27   \\
40 & 12 & 6.4e12 & 3.5e24 &  2.0e36\\
50 & 12 & 6.5e15 & 3.7e30 & 2.1e45 \\
100 & 12 & 3.4e21 & 4.7e60  & 3.0e90  \\
\bottomrule
% \hspace{0.4\columnwidth}
\end{tabular}
% \vspace{-12pt}
\end{threeparttable}
\Caption{Values of $\hammerlimit$ by $\dimnumber$ and $\rratio$ for $\epsilon=10^{-5}$ from \Cref{eq:m_in_n}.}
{
\liyi{(January 20, 2014) Do we really need a table to show values of an analytical function? If showing data points is really warranted, I suggest plotting curves instead of tabulation, much more intuitive and better looking.
Also, I merged the two tables together to avoid duplication.
I think appendix is a much better place.
}%liyi
\scott{graph added to body. the nice thing about the table is it emphasizes the invariance of the first column.}
} 
\label{tab:m_div_n_body}
\label{tab:m_div_n}
\end{table}


==> motion_planning_fig.tex <==
\begin{figure}[tbh]
  \centering
  \includegraphics[width=\linewidth]{figs/motionplanning/hrp4.png}
  \Caption{23D robot motion planning}
  {
  }
  \label{fig:teaser_motion_planning}
\end{figure}


==> mps_maximality_fig.tex <==
\begin{figure*}
\centering
  \subfloat[d = 4]{
     \label{fig:mps_maximality_4d}
     \includegraphics[width=0.24\linewidth]{figs/MPS_4d_new.pdf}
  }    
  \subfloat[d = 6]
  { \label{fig:mps_maximality_6d}
     \includegraphics[width=0.24\linewidth]{figs/MPS_6d_new.pdf}
  }  
  \subfloat[d = 8]
  { \label{fig:mps_maximality_8d}
     \includegraphics[width=0.24\linewidth]{figs/MPS_8d_new.pdf} 
  }
  \subfloat[d = 10]
  { \label{fig:mps_maximality_10d}
     \includegraphics[width=0.24\linewidth]{figs/MPS_10d_new.pdf} 
  }
 \Caption{Number of points $\samplenumber$ generated by different methods across dimension.}{We are capable of generating large distributions in high dimensions.}
 \label{fig:mps_maximality}
\end{figure*}
%[tbh]

\nothing{
\mohamed{Degen Plane Spokes Rocks! }
\Spokesearch{} using short spoke darts approach maximality much faster than Line darts, as measured by the number of inserted points in a given run time. While being the most affordable methods that one can use to solve the MPS methods in $d \ge 6$, Line darts and Spoke darts with our proposed \spokesearch{} method require significantly larger time to approach maximality as the number of dimensions increases.
\liyi{(December 25, 2013) Please trim all pdf figures in a consistent fashion so that they have the same sizes. \subref{fig:mps_maximality_6d} is better as it has no wasted margin.}
\liyi{(December 25, 2013) There are missing curves in some of the figures. Also, looks like we should add \emacsquote{plane darts} for symmetry since we have plane spokes.}
\mohamed{These are unfinished figures, the entire set will be updated after Chonhyon finish his experiments using my code and his GPU code. The purpose of these results is to demonstrate the superiority of spoke darts according to the few experiments I have done on my machine. Chonhyon will do the full set of experiments and update this figure. The right 2 figure are copied of $d = 4$ anyways :D}

\liyi{(Jaunary 16, 2014) There is a 6th green curve in each plot; what is that?}
}%nothing


==> plane_spoke_alg.tex <==
\begin{algorithm}
  \Caption{Trim wheel, for dense blue noise.}{}
  \label{alg:trim_wheel}
  \begin{algorithmic} [1]
    \REQUIRE input plane spoke $\planespoke \supset \{a,b\}$ for sample $\sample$
    \ENSURE trimmed line spoke $\linespokeprime \subset \planespoke$
    \STATE $p \leftarrow $ Trim anchor point($a$)
    \IF{ $p$ = empty}
      \STATE arc $\linespoke \leftarrow$ Trim all segments ( circle through $a$ and $b$ )
      \STATE $p \leftarrow $ RandomSample( longest $\linespoke$ )
    \ENDIF        
    \STATE $\linespoke \leftarrow $ line$(\sample, p)$
    \STATE $\linespokeprime \leftarrow$ Trim anchored segment( $\linespoke$, $p$ )
    \RETURN\ $\linespokeprime$
  \end{algorithmic}
\end{algorithm}


==> proof_hid.tex <==
%\section{Bound Proofs for Section~\protect\ref{sec:parameters}}
\section{Bound Proofs}
\label{sec:boundproofs}

\liyi{I unwrap the single subsection. There are a whole bunch of naked symbols here but I don't have time to fix.}
\scott{I fixed the rest}

%=================================================================
%\subsection{Bound on Missed Throws $\hammerlimit$, in $\rratio$, $\dimnumber$, and $\bigbetachance$}
\label{sec:randomized_coverage}
Here we prove the bounds on $\hammerlimit$, $\rratio$, and $\bigbetachance$ in terms of $\dimnumber$ 
from \Cref{sec:parameters}. 
\note{Here we only consider constant-radius balls.}
%
%def
A \emph{void} is an uncovered region. It is bounded by some disks.
The chance of hitting a void will depend on its \emph{surface area} 
$\area(\void)$, the $\dimnumber$-1 dimensional volume of its boundary.
It will also depend on the surface area of any disk on its boundary, $\area(\disk)$.
We first consider \linespokesalg.

\subsection{Chance of missing the void from one disk}
Let us quantify the chance $\pmissi{1}$ that a \linespoketext{} from disk $\disk_1$ missed a void.
See \Cref{fig:shared_area}.
Let $\vdarearatio_1 =  \area(\void \cap \disk_1) / \area( \disk_1 ).$
Since line-spokes are chosen uniformly from the surface area of the disk,
$\phiti{1} = \vdarearatio_1,$ and $\pmissi{1} = 1 - \vdarearatio_1.$
%(We may multiply the hit chance by 2 if the extent of the void is small enough that it does not contain antipodal points of the disk and we use a line rather than a ray for a spoke.)

The chance of missing $\hammerlimit$ times consecutively is then
$\pmissmi{1} = \prod_{j=1}^{\hammerlimit} (1 - \vdarearatio_1) = (1 - \vdarearatio_1)^\hammerlimit.$
Using the well-known inequality $e^{-x} = \exp(-x) > 1 -x,$ we have 
$\pmissmi{1} < \exp(-\hammerlimit \vdarearatio_1).$

\subsection{Chance of missing the void from all disks}
\label{sec:all_misses}
The chance of missing $\hammerlimit$ times consecutively from all $\neighbors$ bounding disks is then
$\pmissmi{\textrm{all}} = \prod_{i=1}^\neighbors \pmissmi{i} < \exp\left( -\hammerlimit \sum_{i=1}^\neighbors \vdarearatio_i \right) = \exp( -\hammerlimit \vdarearatio),$
where all sample disks have the same radius and size so we can drop their subscripts and $\vdarearatio = \area(\void) / \area(\disk).$

If we wish this miss chance to be less than $\bigbetachance,$ then it is sufficient to have
$\exp( -\hammerlimit \vdarearatio) < \bigbetachance$
or 
$\hammerlimit \vdarearatio > -\ln( \bigbetachance ) > 0.$

\subsection{Bound in terms of $\rratio$}
Now we bound $\vdarearatio$ in terms of $\rratio.$
Suppose there is a domain point $v$ in the void at distance $\rcoverage$ from all samples.
Then a ball at $v$ of radius $\rvoid = \rcoverage - \rconflict$ is strictly inside the void, and $\area(\void) > \area(\disk(\rvoid));$
see \Cref{fig:ball_void}.
Since we are in $\dimnumber$ dimensions and $\rratio = \rcoverage / \rconflict,$ 
\[\vdarearatio = \frac{\area(\void)}{\area(\disk)} > \frac{\rvoid^{\dimnumber-1}}{\rconflict^{\dimnumber-1}} = (\rratio - 1)^{\dimnumber-1}\]

\scott{There is a huge weakness to this proof and the subsequent bounds. It assumes that the void shape is a ball, and that all the void volume could be in one big connected void. That single-void thing is a global argument that should be a local one. I thought the second-proof would fix that, but the area subtended by a neighboring ball shrinks as the dimension increases, and the numbers I got out of that weren't any better. If only there were good spatial statistics results or I knew that stuff...}

Hence a sufficient condition is 
$\hammerlimit(\rratio-1)^{\dimnumber-1} > - \ln \bigbetachance,$ or

\begin{equation}
   \hammerlimit  = \left\lceil  {(-\ln{\bigbetachance})} (\rratio-1)^{1-\dimnumber} \right\rceil
   \Leftrightarrow
   \rratio = 1 + \left(  \frac{-\ln{\bigbetachance}}{\hammerlimit} \right)^{1/(\dimnumber-1)}
   \label{eq:m_in_n}
\end{equation}


\subsection{Example $\hammerlimit$ Values}

\label{sec:m_div_n_table}
\Cref{tab:m_div_n} gives example $\hammerlimit$ values using \Cref{eq:m_in_n}.
There is considerable slack in the inequalities and we achieve a much smaller $\rratio$ in practice.
 
\input{m_div_n_body_tab}

\subsection{\Twospokesalg}
If the first spoke finds an uncovered point, the second spoke always places a sample, so we need only consider the first spoke.
If we consider the subset of a void that is at least $2r$ from any disk, then the prior analysis shows $\rratio < 4$ within them. The uncovered regions between $r$ and $2r$ have local $\rratio<2$ and are subsumed.
Hence $\hammerlimit=12$ gives $\rratio < 4$ with probability $1 - 10^{-5}.$

\subsection{Subtleties}

\pargrph{Boundary caveats}
The astute reader may have noticed that we made no mention of the domain boundary.
For bounded domains, we assumed that the void was bounded by disks only.
This may be guaranteed by throwing \spokestext{} on or near the domain boundary first.
For periodic domains, several analysis steps are only guaranteed to hold when the void spans less than the domain period. 
We may guarantee that no Voronoi ball spans the period by starting with a few samples well-spaced samples.
Then we need only considering the subset of a void within one domain period.
% two issues: $\area(\void) > \area(\disk(\rvoid))$ is only guaranteed when the void diameter is small compared to the period of the domain. And if the void touches a disk and its periodic copy, only one copy gets to count the 12 successive misses



\pargrph{Order independence}
There is a statistical subtly in \Cref{sec:all_misses}.
It does not matter that the consecutive \spokestext{} from one bounding disk were not consecutive with the \spokestext{} from another disk.
The misses for each of the remaining boundary pieces is independent of whether the void was hit and reduced by some \spokestext{} from a later front disk. 
The important thing is that no \spoketext{} ever hit the boundary of the terminal, remaining void.

% this a note to myself. leave it out of the paper
\scott{
\pargrph{Slack in $1-\vdarearatio_1 < \exp(-\vdarearatio_1)$}
While there is slack in this inequality, it becomes tight in the limit as a void is bounded by an infinite number of balls.
It may be possible to use the kissing number to get a slightly better bound, but the difference will be very small. 
}
%===================
\begin{figure} [!htb] 
 \centering
   
  \subfloat[Shared area of a void and a disk.]
  {
     \includegraphics[height=0.9in]{figs/handdrawn/shared_area_hid.pdf}
     \label{fig:shared_area}
  }%\hspace{12pt}%
%
  \subfloat[An empty ball in a void has smaller area than the void.] %: $\vol(\void) = \vol(\dvoid)$, $\rvoid < \rdvoid$, and $\area(\void) > \area(\dvoid)$.
  {
     \includegraphics[height=0.9in]{figs/handdrawn/ball_void_hid.pdf}
     \label{fig:ball_void}
  }
  \Caption{Hitting a void from a neighboring disk.}
 
 \label{fig::void_by_neighbor}
\end{figure}
%====================

%\subsection{Bound for \inlinespokestext{}}
%The same proof process can be used to obtain a bound on $\rratio$ when using \inlinespokestext{}, but it is weaker by a factor of two.
%Consider a void$^\prime$, the portion of a void outside all $2\rconflict$ disks; and suppose it has a point at distance $\rvoid^{\prime}$ from all $2\rconflict$ disks. Then
%\[\vdarearatio^{\prime} = \frac{\area(\void^\prime)}{\area(2\disk)} > \left(\frac{\rvoid^\prime}{2\rconflict}\right)^{\dimnumber-1} = \left(\frac{\rratio}{2} - 1\right)^{\dimnumber-1},\]
%
%and our sufficient conditions are
%
%\begin{equation}
%   \hammerlimit  = \left\lceil  {(-\ln{\bigbetachance})} \left(\frac{\rratio}{2}-1\right)^{1-\dimnumber} \right\rceil
%   \Leftrightarrow
%   \rratio = 2 + 2\left(  \frac{-\ln{\bigbetachance}}{\hammerlimit} \right)^{1/(\dimnumber-1)}.
%   \label{eq:m_in_n_inward}
%\end{equation}

%\scott{revise this after experiments. I think we will get an even better beta than in the outward spoke case.}



==> ramp_distribution_alg.tex <==
\begin{algorithm}
  \Caption{Sample point from spoke.}{}
  \label{alg:ramp_distribution}
  \begin{algorithmic} [1]
	  \REQUIRE $\linespoke$, an uncovered segment of a trimmed spoke for $\sample$
    \ENSURE $\sampleprime$, a step blue noise sample point 


    \STATE $\linespokeprime \leftarrow \linespokeprime - \disk(\sampleprime)$

    \FOR{each neighbor $\sampleprime$ near $\sample$}
      \IF{$\| a - \sampleprime \|^2 < r^2$}
         \RETURN{} empty %$\linespokeprime$
       \ENDIF
     \ENDFOR       
     \RETURN{} $a$
  \end{algorithmic}
\end{algorithm}


==> rdf_fig.tex <==
% two columns of power and anisotropy
%	\subfloat[MPS]
%	{
%	 }
% Radial distance function and dual radial power for Maximal Poisson-disk Sampling (MPS, traditional blue noise), 


\begin{figure}[tbh]
\centering
	 \subfloat[\Linespokesalg]
	 {
	 \shortstack{ %width=0.3\linewidth
	   \includegraphics[width=0.33\linewidth]{figs/distributions-p-midd/06d/RDFhistogram_337570.png}%\\
	   }
	 }
	 \subfloat[\Favoredspokesalg]
	 {
	 \shortstack{ %width=0.3\linewidth
	   \includegraphics[width=0.33\linewidth]{figs/distributions-p-midd/16d/RDFhistogram_196465.png}%\\
	   }
	 }
	 \subfloat[\Twospokesalg]
	 {
  	   \shortstack{ %width=0.3\linewidth
	   \includegraphics[width=0.33\linewidth]{figs/distributions-p-midd/26d/RDFhistogram_382015.png}%\\
	   }
	 }
 \Caption{RDF's for six dimensional periodic domains.}
 {
 }
 \label{fig:rdf}
\end{figure}

==> rdf_spectra_comparison_fig-new.tex <==
\noindent
\begin{figure*}
	\centering
	\setlength{\tabcolsep}{3pt}
	\resizebox{0.85\linewidth}{!}{
		\begin{tabular}{cccccc}
			\rotatebox[origin=l]{90}{{\color{blue}Point-Annulus}}
			& \includegraphics[height=1in]{figs/bridsonexperiments/2d/fftslice.png}
			& \includegraphics[height=1in]{figs/bridsonexperimentsour/3d/fftslice.png}
			& \includegraphics[height=1in]{figs/bridsonexperimentsour/4d/fftslice.png}
      & \includegraphics[height=1in]{figs/bridsonexperimentsour/5d/fftslice.png}
      & \includegraphics[height=1in]{figs/bridsonexperimentsour/6d/fftslice.png}
			\\
			&\includegraphics[height=1in]{figs/bridsonexperiments/2d/RDFhistogram.png}
			&\includegraphics[height=1in]{figs/bridsonexperimentsour/3d/RDFhistogram.png}
			&\includegraphics[height=1in]{figs/bridsonexperimentsour/4d/RDFhistogram.png}	
      &\includegraphics[height=1in]{figs/bridsonexperimentsour/5d/RDFhistogram.png}
      &\includegraphics[height=1in]{figs/bridsonexperimentsour/6d/RDFhistogram.png}
			\\
      &\includegraphics[height=1in]{figs/bridsonexperiments/2d/radialpower.png}
      &\includegraphics[height=1in]{figs/bridsonexperimentsour/3d/radialpower.png}
			&\includegraphics[height=1in]{figs/bridsonexperimentsour/4d/radialpower.png}
      &\includegraphics[height=1in]{figs/bridsonexperimentsour/5d/radialpower.png}
      &\includegraphics[height=1in]{figs/bridsonexperimentsour/6d/radialpower.png}
			\\
			\rotatebox[origin=l]{90}{{\color{red}Line-Spokes}}
			& \includegraphics[height=1in]{figs/distributions/spoke_spec.png}
			& \includegraphics[height=1in]{figs/distributions-p-midd/03d/slice513_257_80120.png}
			& \includegraphics[height=1in]{figs/distributions-p-midd/04d/slice129_65_61401.png}
      & \includegraphics[height=1in]{figs/distributions-p-midd/05d/slice39_20_6166.png}
      & \includegraphics[height=1in]{figs/distributions-p-midd/06d/slice17_9_337570.png}
      \\
			&\input{figs/distributions/2_P_198_0spoke_411222_beta_points_rdf}
			&\includegraphics[height=1in]{figs/distributions-p-midd/03d/RDFhistogram_80120.png}
			&\includegraphics[height=1in]{figs/distributions-p-midd/04d/RDFhistogram_61401.png}			
			&\includegraphics[height=1in]{figs/distributions-p-midd/05d/RDFhistogram_61401.png}
			&\includegraphics[height=1in]{figs/distributions-p-midd/06d/RDFhistogram_337570.png}
			\\
			&\input{figs/distributions/spoke_rp}
			&\includegraphics[height=1in]{figs/distributions-p-midd/03d/radialpower_80120.png}
		 	&\includegraphics[height=1in]{figs/distributions-p-midd/04d/radialpower_61401.png}
      &\includegraphics[height=1in]{figs/distributions-p-midd/05d/radialpower_6166.png}
      &\includegraphics[height=1in]{figs/distributions-p-midd/06d/radialpower_337570.png}
			\\
			\rotatebox[origin=l]{90}{{\color{magenta}Two-Spokes}}
			& \includegraphics[height=1in]{figs/distributions/two_spec.png}
			& \includegraphics[height=1in]{figs/distributions-p-midd/23d/slice513_257_732051.png}
			& \includegraphics[height=1in]{figs/distributions-p-midd/24d/slice129_65_2214.png}
			& \includegraphics[height=1in]{figs/distributions-p-midd/25d/slice39_20_14088.png}	
			& %\includegraphics[height=1in]{figs/distributions/two_spec.png}
			\\
			&\input{figs/distributions/2_P_397_2two_459569_beta_points_rdf}
			&\includegraphics[height=1in]{figs/distributions-p-midd/23d/RDFhistogram_732051.png}
			&\includegraphics[height=1in]{figs/distributions-p-midd/24d/RDFhistogram_563628.png}
			&\includegraphics[height=1in]{figs/distributions-p-midd/25d/RDFhistogram_452776.png}
			&\includegraphics[height=1in]{figs/distributions-p-midd/26d/RDFhistogram_382015.png}
			\\
			&\input{figs/distributions/two_rp}
			&\includegraphics[height=1in]{figs/distributions-p-midd/23d/radialpower_732051.png}
			&\includegraphics[height=1in]{figs/distributions-p-midd/24d/radialpower_2214.png}
			&\includegraphics[height=1in]{figs/distributions-p-midd/25d/radialpower_14088.png}
			&%\input{figs/distributions/two_rp}
			\\
			\hline
			\\
			&$d=2$ &$d=3$ &$d=4$ &$d=5$ &$d=6$
		\end{tabular}
	}
	\caption{TBD.}
 \label{fig:rdf_spectra_comparison}
\end{figure*}



==> rdf_spectra_comparison_highd_fig.tex <==
{
%\noindent %noindent causes extra vspace when the figure is input
\begin{figure*}
	\centering
	\setlength{\tabcolsep}{3pt}  %2_P_198_0spoke
	\resizebox{0.9\linewidth}{!}{
		\begin{tabular}{ccccccc}
			\multirow{ 3 }{*}{\rotatebox[origin=l]{90}{\textbf{{\color{blue} $\Longleftarrow$ Point-Annulus $\Longrightarrow$}}}}
      & \rotatebox[origin=l]{90}{{\hspace{16pt}spectra}} 
			& \includegraphics[height=1in]{figs/bridsonexperimentsour/10d/fftslice.png}
			& \includegraphics[height=1in]{figs/bridsonexperimentsour/15d/fftslice.png}
			& \includegraphics[height=1in]{figs/bridsonexperimentsour/20d/fftslice.png}
      & \includegraphics[height=1in]{figs/bridsonexperimentsour/25d/fftslice.png}
      & \includegraphics[height=1in]{figs/bridsonexperimentsour/30d/fftslice.png}
			\\
      & \rotatebox[origin=l]{90}{{\hspace{28pt}RDF}}
			&\includegraphics[height=1in]{figs/bridsonexperiments/2d/RDFhistogram.png}
			&\includegraphics[height=1in]{figs/bridsonexperimentsour/3d/RDFhistogram.png}
			&\includegraphics[height=1in]{figs/bridsonexperimentsour/4d/RDFhistogram.png}	
      &\includegraphics[height=1in]{figs/bridsonexperimentsour/5d/RDFhistogram.png}
      &\includegraphics[height=1in]{figs/bridsonexperimentsour/6d/RDFhistogram.png}
			\\
      &\rotatebox[origin=l]{90}{{\hspace{28pt}RP}}
      &\includegraphics[height=1in]{figs/bridsonexperiments/2d/radialpower.png}
      &\includegraphics[height=1in]{figs/bridsonexperimentsour/3d/radialpower.png}
			&\includegraphics[height=1in]{figs/bridsonexperimentsour/4d/radialpower.png}
      &\includegraphics[height=1in]{figs/bridsonexperimentsour/5d/radialpower.png}
      &\includegraphics[height=1in]{figs/bridsonexperimentsour/6d/radialpower.png}
			\\
			\hline
			\\
			\multirow{ 3 }{*}{\rotatebox[origin=l]{90}{\textbf{{\color{red} $\Longleftarrow$ Line-Spokes $\Longrightarrow$}}}}
      &\rotatebox[origin=l]{90}{{\hspace{16pt}spectra}}
%			& \includegraphics[height=1in]{figs/distributions/spoke_spec.png}
			& \includegraphics[height=1in]{figs/distributions-p-midd/010d/fftslice.png}
			& \includegraphics[height=1in]{figs/distributions-p-midd/015d/fftslice.png}
			& \includegraphics[height=1in]{figs/distributions-p-midd/020d/fftslice.png}
 		        & \includegraphics[height=1in]{figs/distributions-p-midd/025d/fftslice.png}
		        & \includegraphics[height=1in]{figs/distributions-p-midd/030d/fftslice.png}
      \\
      &\rotatebox[origin=l]{90}{{\hspace{28pt}RDF}}
%			&\input{figs/distributions/2_P_198_0spoke_411222_beta_points_rdf}
			&\includegraphics[height=1in]{figs/distributions-p-midd/010d/RDFhistogram.png}
			&\includegraphics[height=1in]{figs/distributions-p-midd/015d/RDFhistogram.png}
			&\includegraphics[height=1in]{figs/distributions-p-midd/020d/RDFhistogram.png}			
			&\includegraphics[height=1in]{figs/distributions-p-midd/025d/RDFhistogram.png}
			&\includegraphics[height=1in]{figs/distributions-p-midd/030d/RDFhistogram.png}
			\\
      &\rotatebox[origin=l]{90}{{\hspace{28pt}RP}}
%			&\input{figs/distributions/spoke_rp}
			&\includegraphics[height=1in]{figs/distributions-p-midd/010d/radialpower.png}
			&\includegraphics[height=1in]{figs/distributions-p-midd/015d/radialpowerpng}
		 	&\includegraphics[height=1in]{figs/distributions-p-midd/020d/radialpower.png}
     	 		&\includegraphics[height=1in]{figs/distributions-p-midd/025d/radialpower.png}
      			&\includegraphics[height=1in]{figs/distributions-p-midd/030d/radialpower.png}
			\\
			\hline
			\\
			\multirow{ 3 }{*}{\rotatebox[origin=l]{90}{\textbf{{\color{magenta} $\Longleftarrow$ Two-Spokes $\Longrightarrow$}}}}
      &\rotatebox[origin=l]{90}{{\hspace{16pt}spectra}} 
%			& \includegraphics[height=1in]{figs/distributions/two_spec.png}
			& \includegraphics[height=1in]{figs/distributions-p-midd/210d/fftslice.png}
			& \includegraphics[height=1in]{figs/distributions-p-midd/215d/fftslice.png}
			& \includegraphics[height=1in]{figs/distributions-p-midd/220d/fftslice.png}
           		& \includegraphics[height=1in]{figs/distributions-p-midd/225d/fftslice.png}  
            		& \includegraphics[height=1in]{figs/distributions-p-midd/230d/fftslice.png}
			\\
      &\rotatebox[origin=l]{90}{{\hspace{28pt}RDF}}
%			&\input{figs/distributions/2_P_397_2two_459569_beta_points_rdf}
			&\includegraphics[height=1in]{figs/distributions-p-midd/22d/RDFhistogram_8118176.png}
			&\includegraphics[height=1in]{figs/distributions-p-midd/23d/RDFhistogram_732051.png}
			&\includegraphics[height=1in]{figs/distributions-p-midd/24d/RDFhistogram_563628.png}
			&\includegraphics[height=1in]{figs/distributions-p-midd/25d/RDFhistogram_452776.png}
			&\includegraphics[height=1in]{figs/distributions-p-midd/26d/RDFhistogram_382015.png}
			\\
      &\rotatebox[origin=l]{90}{{\hspace{28pt}RP}}
%			&\input{figs/distributions/two_rp}
			&\includegraphics[height=1in]{figs/distributions-p-midd/22d/radialpower_1913.png}
			&\includegraphics[height=1in]{figs/distributions-p-midd/23d/radialpower_732051.png}
			&\includegraphics[height=1in]{figs/distributions-p-midd/24d/radialpower_2214.png}
		    &\includegraphics[height=1in]{figs/distributions-p-midd/25d/radialpower_14088.png}
            &\includegraphics[height=1in]{figs/distributions-p-midd/26d/radialpower_54468.png}
			\\
			\hline
			\\
			& &$\dimnumber=10$ &$\dimnumber=15$ &$\dimnumber=20$ &$\dimnumber=25$ &$\dimnumber=30$
		\end{tabular}
	}
	\Caption{Spectra, RDF, and RP of methods by dimension. Anisotropy is negligible. In RDF, ``1'' is scaled to $r$, the sampling radius.}
        {%
        }
 \label{fig:rdf_spectra_comparison}
\end{figure*}
}

==> rdf_spectra_fig.tex <==
% spectra in dimensions 3-4-5 by all three algorithms

\begin{figure}[tbh]
\centering
	 \subfloat[$d=3$]
	 {
	 \shortstack{ %width=0.3\linewidth
	   \includegraphics[height=0.8in]{figs/distributions-p-midd/03d/slice513_257_80120.png}\\
  	   \includegraphics[height=0.8in]{figs/distributions-p-midd/03d/RDFhistogram_80120.png}\\
  	   \includegraphics[height=0.8in]{figs/distributions-p-midd/03d/radialpower_80120.png}\\
  	   \includegraphics[height=0.8in]{figs/distributions-p-midd/03d/radialisotropy_80120.png}
	   }
	 }
	 \subfloat[$d=4$]
	 {
	 \shortstack{ %width=0.3\linewidth
	   \includegraphics[height=0.8in]{figs/distributions-p-midd/04d/slice129_65_61401.png}\\
	   \includegraphics[height=0.8in]{figs/distributions-p-midd/04d/RDFhistogram_61401.png}\\
  	   \includegraphics[height=0.8in]{figs/distributions-p-midd/04d/radialpower_61401.png}\\
  	   \includegraphics[height=0.8in]{figs/distributions-p-midd/04d/radialisotropy_61401.png}
	   }
	 }
	 \subfloat[$d=5$]
	 {
	 \shortstack{ %width=0.3\linewidth
	   \includegraphics[height=0.8in]{figs/distributions-p-midd/05d/slice39_20_6166.png}\\
	   \includegraphics[height=0.8in]{figs/distributions-p-midd/05d/RDFhistogram_61401.png}\\
  	   \includegraphics[height=0.8in]{figs/distributions-p-midd/05d/radialpower_6166.png}\\
  	   \includegraphics[height=0.8in]{figs/distributions-p-midd/05d/radialisotropy_6166.png}
	   }
	 }
 \caption{\Linespokesalg\ spectra in higher dimensions.}
 \label{fig:rdf_spectra_ld}
\end{figure}


\begin{figure}[tbh]
\centering
	 \subfloat[$d=3$]
	 {
	 \shortstack{ %width=0.3\linewidth
	   \includegraphics[height=0.8in]{figs/distributions-p-midd/13d/slice513_257_128835.png}\\
  	   \includegraphics[height=0.8in]{figs/distributions-p-midd/13d/RDFhistogram_128835.png}\\
  	   \includegraphics[height=0.8in]{figs/distributions-p-midd/13d/radialpower_128835.png}\\
  	   \includegraphics[height=0.8in]{figs/distributions-p-midd/13d/radialisotropy_128835.png}
	   }
	 }
	 \subfloat[$d=4$]
	 {
	 \shortstack{ %width=0.3\linewidth
	   \includegraphics[height=0.8in]{figs/distributions-p-midd/14d/slice129_65_172646.png}\\
	   \includegraphics[height=0.8in]{figs/distributions-p-midd/14d/RDFhistogram_172646.png}\\
  	   \includegraphics[height=0.8in]{figs/distributions-p-midd/14d/radialpower_172646.png}\\
  	   \includegraphics[height=0.8in]{figs/distributions-p-midd/14d/radialisotropy_172646.png}
	   }
	 }
	 \subfloat[$d=5$]
	 {
	 \shortstack{ %width=0.3\linewidth
	   \includegraphics[height=0.8in]{figs/distributions-p-midd/15d/slice39_20_251358.png}\\
	   \includegraphics[height=0.8in]{figs/distributions-p-midd/15d/RDFhistogram_251358.png}\\
  	   \includegraphics[height=0.8in]{figs/distributions-p-midd/15d/radialpower_251358.png}\\
  	   \includegraphics[height=0.8in]{figs/distributions-p-midd/15d/radialisotropy_251358.png}
	   }
	 }
 \caption{\Favoredspokesalg\ spectra in higher dimensions.}
 \label{fig:rdf_spectra_fd}
\end{figure}


\begin{figure}[tbh]
\centering
	 \subfloat[$d=3$]
	 {
	 \shortstack{ %width=0.3\linewidth
	   \includegraphics[height=0.8in]{figs/distributions-p-midd/23d/slice513_257_732051.png}\\
  	   \includegraphics[height=0.8in]{figs/distributions-p-midd/23d/RDFhistogram_732051.png}\\
  	   \includegraphics[height=0.8in]{figs/distributions-p-midd/23d/radialpower_732051.png}\\
  	   \includegraphics[height=0.8in]{figs/distributions-p-midd/23d/radialisotropy_732051.png}
	   }
	 }
	 \subfloat[$d=4$]
	 {
	 \shortstack{ %width=0.3\linewidth
	   \includegraphics[height=0.8in]{figs/distributions-p-midd/24d/slice129_65_563628.png}\\
	   \includegraphics[height=0.8in]{figs/distributions-p-midd/24d/RDFhistogram_563628.png}\\
  	   \includegraphics[height=0.8in]{figs/distributions-p-midd/24d/radialpower_563628.png}\\
  	   \includegraphics[height=0.8in]{figs/distributions-p-midd/24d/radialisotropy_563628.png}
	   }
	 }
	 \subfloat[$d=5$]
	 {
	 \shortstack{ %width=0.3\linewidth
	   \includegraphics[height=0.8in]{figs/distributions-p-midd/25d/slice39_20_452776.png}\\
	   \includegraphics[height=0.8in]{figs/distributions-p-midd/25d/RDFhistogram_452776.png}\\
  	   \includegraphics[height=0.8in]{figs/distributions-p-midd/25d/radialpower_452776.png}\\
  	   \includegraphics[height=0.8in]{figs/distributions-p-midd/25d/radialisotropy_452776.png}
	   }
	 }
 \caption{\Twospokesalg\ spectra in higher dimensions.}
 \label{fig:rdf_spectra_ld}
\end{figure}

%\begin{figure}[tbh]
%\centering	 
%	 % original, unmodified versions
%	   \input{figs/distributions/2_P_198_0spoke_411222_beta_points_rp}
%	   \input{figs/distributions/2_P_281_1favored_384057_beta_points_rp}
% 	   \input{figs/distributions/2_P_397_2two_459569_beta_points_rp}
%\end{figure}
	 


==> rdf_spectra_teaser_fig.tex <==
% two columns of power and anisotropy
%	\subfloat[MPS]
%	{
%	 }
% Radial distance function and dual radial power for Maximal Poisson-disk Sampling (MPS, traditional blue noise), 


\begin{figure}[bt]
\centering
	 \subfloat[\Linespokesalg]
	 {
	 \shortstack{ %width=0.3\linewidth
	   \includegraphics[height=1in]{figs/distributions/2_P_24_0spoke_6236_final-half_plot_2d_no_ghosts.pdf}\\
	   \includegraphics[height=1in]{figs/distributions/spoke_spec.png}\\
	   \input{figs/distributions/2_P_198_0spoke_411222_beta_points_rdf}\\
  	   \input{figs/distributions/spoke_rp}
	   }
	 }
	 \subfloat[\Favoredspokesalg]
	 {
	 \shortstack{
	   \includegraphics[height=1in]{figs/distributions/2_P_24_1favored_2949_final-half_plot_2d_no_ghosts.pdf}\\
	   \includegraphics[height=1in]{figs/distributions/favored_spec.png}\\
	   \input{figs/distributions/2_P_281_1favored_384057_beta_points_rdf}\\
	   \input{figs/distributions/favored_rp}
	   }
	 }
	 \subfloat[\Twospokesalg]
	 {
	 \shortstack{
	   \includegraphics[height=1in]{figs/distributions/2_P_24_2two_1631_final-half_plot_2d_no_ghosts.pdf}\\
	   \includegraphics[height=1in]{figs/distributions/two_spec.png}\\
	   \input{figs/distributions/2_P_397_2two_459569_beta_points_rdf}\\
	   \input{figs/distributions/two_rp}
	   }
	 }
 \caption{Example periodic distributions and spectra for our spoke-dart sampling variations. Samples are chosen from a local neighborhood around a prior sample, but the three different rules result in different packing densities and spectra. Top: point sets with the same $r,$ where solid circles of radius $r/2$ do not overlap. Second: periodogram, the Fourier transform of the point sets. Third: Radial Distance Function (RDF), the histogram of pairwise distances between points, with $r=1$. Fourth: Radial Power (RP), the radial average of the periodogram, the dual of the RDF.}
 \label{fig:rdf_spectra_teaser}
\end{figure}

%\begin{figure}[tbh]
%\centering	 
%	 % original, unmodified versions
%	   \input{figs/distributions/2_P_198_0spoke_411222_beta_points_rp}
%	   \input{figs/distributions/2_P_281_1favored_384057_beta_points_rp}
% 	   \input{figs/distributions/2_P_397_2two_459569_beta_points_rp}
%\end{figure}
	 


==> rebuttal_sig14.tex <==
\section{Rebuttal}
\label{sec:rebuttal}

\note{1000 word limit}

Dear reviewers:
Thank you for your careful reading and suggestions. You noted that the paper has novel ideas, simple and yet solid algorithms, useful analysis, and interesting applications. 

* Main issues *

Q: Suitability for graphics (R2, R4, R22)

Our core contribution, the idea of spoke darts and derived algorithms, are extended from sampling algorithms in computer graphics. Thus, we consider this to be a graphics algorithm paper with diverse applications in geometry, optimization, and robotics.

The SIGGRAPH 2014 technical papers CFP specifically asks for submissions that "stimulate trends" and "encourage submissions from areas related to computer graphics, including ... computer aided design, ... robotics, ... the list is not exhaustive."
High-dimensional optimization of multi-parameter geometric designs ties to computer aided design.
Other potential core applications of high-dimensional sampling, such as rendering, are certainly worth pursuing but beyond the scope of our paper.

\scott{In a prior version, I also said the CFP asks for computer aided design. My thinking was that optimization and Delaunay graphs are common parts of computer aided design, depending on how you defined computer aided design. I'll leave it to you Li-Yi to decide whether to add computer aided design back in, with the explanation that our other two applications tie to the CFP. One virtue of adding it back is that then all three of our applications have a direct tie to the CFP. Actually, that is a nice wording IMO: "All three of our applications have a direct tie to the CFP. Delaunay graphs and optimization are common components of computer aided design."}
\liyi{Good point. I didn't know this connection and that is why I removed it. However, does computer aided design usually need *high dimensional* optimization and Delaunay graph? If not, it might not benefit us to mention it, as reviewers might think we don't know what we are talking about.}
\scott{High-dimensional design optimization ``yes,'' high-dimensional Delaunay graph ``no.'' How about I mention ``ties'' so that they realize we realize the connection may not be direct. Do you like the above reworking?}
\liyi{OK, as a native speaker, you know more about exact English work play than me.}

We believe SIGGRAPH, with its unique diversity, is the best venue to share a sampling paper with diverse applications. 
We know of no better venue.

SIGGRAPH has a long history of benefiting from ideas from other fields, as diverse as physics, perception, and biology. 
We would like to demonstrate that graphics algorithms can also benefit other fields.

Q: [Bridson 2007] Fast Poisson-disk sampling in arbitrary dimensions (R4, R47, R88)

A: We regret omitting Bridson. We know the paper, and agree we must reference and discuss in revision. In brief, point sampling from the annulus suffers from the curse of dimensionality. Bridson does not suggest how many samples are adequate to achieve any level of saturation, but a quick volume analysis following our proof style shows that $O(2^d)$ samples are needed for something like beta=2, independent of a background grid.

Data on Bridson actually makes the case that high-dimensional Poisson-disk sampling is important to SIGGRAPH. Bridson is only a single-page sketch, with many omitted details. Despite this, it has been cited 44 times: 9 TOG, 4 CGF, 17 CG applications such as rendering, and 11 bio/cognition/VR/sensors/signals publications.
Our paper is the first practical version for high dimensional sampling, and we think the SIGGRAPH audience would be interested.

* Other points *

Q: Any 'important' Lipschitz graphics functions? (R64)

A: Some examples follow: distances including geodesics, intensities from non-point sources, power spectra, sound fields, fluid velocity fields, temperature fields. Since our algorithm handles arbitrary and unknown Lipschitz constants, pretty much anything continuous, or piecewise continuous, works.

Q: Lack of power and anisotropy analysis (R2, R47)

A: We have excellent anisotropy because full line spokes have isotropic directions. 
An earlier draft included 2-d plots, but we removed them to focus on high dimensions. We will re-include them.
As described in the paper, we use DDA instead of Fourier spectra because it is more efficient and can effectively detect artifacts.

Q: Plane spokes not uniform from annulus (R4); Worm-patterns (R47) of tight packing (R4).

A: Our implementation of plane-spokes is not uniform sampling, as it has more points at distance exactly r; figure 5a.
We chose this for efficiency, driven by our applications.
One may uniformly sample from a plane-spoke annulus, a 2-d problem, using [Ebeida et al. 2011].
We will revise the introduction to make this direction clear.

\liyi{I removed the opening *correct* as otherwise we are admitting worm patterns.}

Q: Well-spaced samples not efficient for integration in d $>$ 7. (R22)

A: Perhaps true for integration. However, for interpolation, ``no large gaps'' improves accuracy, and ``no close pairs'' reduces noise, in all dimensions.


Q: Novelty over k-d darts [Ebeida et al. 2014]; Why "spoke-darts ... in small gaps ...?" (R88)

A: k-d darts does *global*, axis-aligned hyperplanes. 
Spoke-darts does *local*, radially-aligned hyperplanes.
Radial directions are more efficient for spherical neighborhoods.

Locality provides local saturation bounds.
To ensure that a gap has radius $<$ r, k-d darts requires $O((1/r)^d)$ missed samples. Spoke-darts only requires 12, regardless of r and d.

Q: Comparing to QHull unfair; Algorithm 4 produces exact Delaunay graph? (R88)

A: 
Yes, we compare an exact and an approximate algorithm. We have few alternatives as explained in the section. 
Algorithm 4 produces a subset of edges but converges to the full graph as the number of samples approaches infinity.

Q: Effect of missing Delaunay graph edges on applications? (R47)

A: Even with many missing edges, the extra Voronoi cell volume subtends a small solid angle at the sample point, so it is  small, or narrow-and-far.
We cannot answer how all applications that could use a Delaunay graph are affected by an approximate version, mainly because high dimensional applications currently work around the Delaunay graph because, until our paper, there was no way to get a useful approximate subset in sub-exponential time, e.g. DIRECT uses rectangle diagonals, informatics uses k-nearest neighbors.
A close analogy is that nearest-neighbor queries in high dimensions have long relied on approximate answers, which are the only answers available in sub-linear time.

\liyi{narrow and *far*? what does this term mean anyway?}
\scott{subtends a small solid angle. If it is big, then it must be far away from the sample point. I added more explanation above.}

Q: Global opt: separate paper, more tests (R22)

A: Feedback from global optimization experts: most important contribution is better sample neighborhoods and size estimation.  They say test functions are always anecdotal, and may not cover any given problem domain. Here we emphasize the versatile utility of spoke-darts.
\note{skip, as it doesn't help: We plan a follow-on paper to an optimization journal.}


Q: Performance scaling (R22)

A:  Memory is $O(d n),$ and beta=2 runtime is $O(d n^2),$ both linear in d. 
Linear memory in n means 1,000,000 points in any d is possible;
quadratic time in n means it requires patience.

\note{ skip, they didn't ask: The dependence of n on r, d, and the domain size has no easy answer, and is studied in lattice-theory.}


Q: k-dtree implies curse of dimensionality? (R47)

A: Our k-d tree implementation devolves to ``all samples are neighbors'' and $O(dn)$ query time.

Q: Algorithm difference, speedup over, [Park et al. 2013] (R88)

A: Both use precomputed Poisson-disk samples, for parallel route exploration.  Both use the same adaptive sampling and RRT algorithm; no speedup expected. 
The key is that [Park et al. 2013] is limited to 6 DOF, while our method enables 23 DOF and practical parallel RRT in that space.

QA: We will expand limitations in revision. (R88,R22)

\scott{skip unless we have an answer. We did discuss some limitations so I don't know why they said none provided.}


\scott{==== 1000 word boundary ====}

%---
\scott{very low priority items here, probably beyond 1000 words}

%---

Q: Missing reference [Heck et al.\ 2013] on blue noise vs.\ Poisson-disk (R22).

A: Agreed, will include.

%----


Q: Delaunay graph and optimization uses spoke-darts but not the main algorithm. (R47)

A: This is correct. We think it is a strength that spoke-darts are versatile, and can solve sampling problems without going through the intermediate step of generating well-spaced point samples.

%----

\scott{skip. We don't have an answer yet, and it is new experiments.}
Q: \#points \textless 150,000 (R22)

A: beta=2, d=10, \#points= 1,000,000 took xxx seconds.

%---


%----
\scott{skip unless we have an answer. We did discuss some limitations so I don't know why they said none provided.}
Q: Limitations not discussed (R4, R88,R22)

A: ?? 
%----
=======
\section{Rebuttal (SIGGRAPH 2014)}
\label{sec:rebuttal_sig14}

\note{1000 word limit}

Dear reviewers:
Thank you for your careful reading and suggestions. You noted that the paper has novel ideas, simple and yet solid algorithms, useful analysis, and interesting applications. 

* Main issues *

Q: Suitability for graphics (R2, R4, R22)

Our core contribution, the idea of spoke darts and derived algorithms, are extended from sampling algorithms in computer graphics. Thus, we consider this to be a graphics algorithm paper with diverse applications in geometry, optimization, and robotics.

The SIGGRAPH 2014 technical papers CFP specifically asks for submissions that "stimulate trends" and "encourage submissions from areas related to computer graphics, including ... computer aided design, ... robotics, ... the list is not exhaustive."
High-dimensional optimization of multi-parameter geometric designs ties to computer aided design.
Other potential core applications of high-dimensional sampling, such as rendering, are certainly worth pursuing but beyond the scope of our paper.

\scott{In a prior version, I also said the CFP asks for computer aided design. My thinking was that optimization and Delaunay graphs are common parts of computer aided design, depending on how you defined computer aided design. I'll leave it to you Li-Yi to decide whether to add computer aided design back in, with the explanation that our other two applications tie to the CFP. One virtue of adding it back is that then all three of our applications have a direct tie to the CFP. Actually, that is a nice wording IMO: "All three of our applications have a direct tie to the CFP. Delaunay graphs and optimization are common components of computer aided design."}
\liyi{Good point. I didn't know this connection and that is why I removed it. However, does computer aided design usually need *high dimensional* optimization and Delaunay graph? If not, it might not benefit us to mention it, as reviewers might think we don't know what we are talking about.}
\scott{High-dimensional design optimization ``yes,'' high-dimensional Delaunay graph ``no.'' How about I mention ``ties'' so that they realize we realize the connection may not be direct. Do you like the above reworking?}
\liyi{OK, as a native speaker, you know more about exact English work play than me.}

We believe SIGGRAPH, with its unique diversity, is the best venue to share a sampling paper with diverse applications. 
We know of no better venue.

SIGGRAPH has a long history of benefiting from ideas from other fields, as diverse as physics, perception, and biology. 
We would like to demonstrate that graphics algorithms can also benefit other fields.

Q: [Bridson 2007] Fast Poisson-disk sampling in arbitrary dimensions (R4, R47, R88)

A: We regret omitting Bridson. We know the paper, and agree we must reference and discuss in revision. In brief, point sampling from the annulus suffers from the curse of dimensionality. Bridson does not suggest how many samples are adequate to achieve any level of saturation, but a quick volume analysis following our proof style shows that $O(2^d)$ samples are needed for something like beta=2, independent of a background grid.

Data on Bridson actually makes the case that high-dimensional Poisson-disk sampling is important to SIGGRAPH. Bridson is only a single-page sketch, with many omitted details. Despite this, it has been cited 44 times: 9 TOG, 4 CGF, 17 CG applications such as rendering, and 11 bio/cognition/VR/sensors/signals publications.
Our paper is the first practical version for high dimensional sampling, and we think the SIGGRAPH audience would be interested.

* Other points *

Q: Any 'important' Lipschitz graphics functions? (R64)

A: Some examples follow: distances including geodesics, intensities from non-point sources, power spectra, sound fields, fluid velocity fields, temperature fields. Since our algorithm handles arbitrary and unknown Lipschitz constants, pretty much anything continuous, or piecewise continuous, works.

Q: Lack of power and anisotropy analysis (R2, R47)

A: We have excellent anisotropy because full line spokes have isotropic directions. 
An earlier draft included 2-d plots, but we removed them to focus on high dimensions. We will re-include them.
As described in the paper, we use DDA instead of Fourier spectra because it is more efficient and can effectively detect artifacts.

Q: Plane spokes not uniform from annulus (R4); Worm-patterns (R47) of tight packing (R4).

A: Our implementation of plane-spokes is not uniform sampling, as it has more points at distance exactly r; figure 5a.
We chose this for efficiency, driven by our applications.
One may uniformly sample from a plane-spoke annulus, a 2-d problem, using [Ebeida et al. 2011].
We will revise the introduction to make this direction clear.

\liyi{I removed the opening *correct* as otherwise we are admitting worm patterns.}

Q: Well-spaced samples not efficient for integration in d $>$ 7. (R22)

A: Perhaps true for integration. However, for interpolation, ``no large gaps'' improves accuracy, and ``no close pairs'' reduces noise, in all dimensions.


Q: Novelty over k-d darts [Ebeida et al. 2014]; Why "spoke-darts ... in small gaps ...?" (R88)

A: k-d darts does *global*, axis-aligned hyperplanes. 
Spoke-darts does *local*, radially-aligned hyperplanes.
Radial directions are more efficient for spherical neighborhoods.

Locality provides local saturation bounds.
To ensure that a gap has radius $<$ r, k-d darts requires $O((1/r)^d)$ missed samples. Spoke-darts only requires 12, regardless of r and d.

Q: Comparing to QHull unfair; Algorithm 4 produces exact Delaunay graph? (R88)

A: 
Yes, we compare an exact and an approximate algorithm. We have few alternatives as explained in the section. 
Algorithm 4 produces a subset of edges but converges to the full graph as the number of samples approaches infinity.

Q: Effect of missing Delaunay graph edges on applications? (R47)

A: Even with many missing edges, the extra Voronoi cell volume subtends a small solid angle at the sample point, so it is  small, or narrow-and-far.
We cannot answer how all applications that could use a Delaunay graph are affected by an approximate version, mainly because high dimensional applications currently work around the Delaunay graph because, until our paper, there was no way to get a useful approximate subset in sub-exponential time, e.g. DIRECT uses rectangle diagonals, informatics uses k-nearest neighbors.
A close analogy is that nearest-neighbor queries in high dimensions have long relied on approximate answers, which are the only answers available in sub-linear time.

\liyi{narrow and *far*? what does this term mean anyway?}
\scott{subtends a small solid angle. If it is big, then it must be far away from the sample point. I added more explanation above.}

Q: Global opt: separate paper, more tests (R22)

A: Feedback from global optimization experts: most important contribution is better sample neighborhoods and size estimation.  They say test functions are always anecdotal, and may not cover any given problem domain. Here we emphasize the versatile utility of spoke-darts.
\note{skip, as it doesn't help: We plan a follow-on paper to an optimization journal.}


Q: Performance scaling (R22)

A:  Memory is $O(d n),$ and beta=2 runtime is $O(d n^2),$ both linear in d. 
Linear memory in n means 1,000,000 points in any d is possible;
quadratic time in n means it requires patience.

\note{ skip, they didn't ask: The dependence of n on r, d, and the domain size has no easy answer, and is studied in lattice-theory.}


Q: k-dtree implies curse of dimensionality? (R47)

A: Our k-d tree implementation devolves to ``all samples are neighbors'' and $O(dn)$ query time.

Q: Algorithm difference, speedup over, [Park et al. 2013] (R88)

A: Both use precomputed Poisson-disk samples, for parallel route exploration.  Both use the same adaptive sampling and RRT algorithm; no speedup expected. 
The key is that [Park et al. 2013] is limited to 6 DOF, while our method enables 23 DOF and practical parallel RRT in that space.

QA: We will expand limitations in revision. (R88,R22)

\scott{skip unless we have an answer. We did discuss some limitations so I don't know why they said none provided.}


\scott{==== 1000 word boundary ====}

%---
\scott{very low priority items here, probably beyond 1000 words}

%---

Q: Missing reference [Heck et al.\ 2013] on blue noise vs.\ Poisson-disk (R22).

A: Agreed, will include.

%----


Q: Delaunay graph and optimization uses spoke-darts but not the main algorithm. (R47)

A: This is correct. We think it is a strength that spoke-darts are versatile, and can solve sampling problems without going through the intermediate step of generating well-spaced point samples.

%----

\scott{skip. We don't have an answer yet, and it is new experiments.}
Q: \#points \textless 150,000 (R22)

A: beta=2, d=10, \#points= 1,000,000 took xxx seconds.

%---


%----
\scott{skip unless we have an answer. We did discuss some limitations so I don't know why they said none provided.}
Q: Limitations not discussed (R4, R88,R22)

A: ?? 
%----


==> scaling_method_fig.tex <==

\begin{figure}[tbh]
  \centering
   \subfloat[Neighbor scaling]
   {
      \label{fig:neighbors_by_d}
       \includegraphics[width=0.5\linewidth]{figs/scaling/neighbors_by_d.pdf}
    }
   \subfloat[Time and $n$ scaling]
   {
     \label{fig:}
       \includegraphics[width=0.5\linewidth]{figs/scaling/.pdf}
    }
   \caption{%
\Favoredspokesalg\ and \twospokesalg\ ratios over \linespokesalg, using $k$-d trees over periodic domains. For fixed $\samplenumber$, favored- and two- take a small constant factor longer than \linespokesalg, mainly due to their larger search neighborhoods. For fixed disk radius $r$, favored- and two- produce a constant factor fewer disks $n$. These factors and the number of neighbors $N$ are exponential in dimension, consistent with the ratio of the volume of spheres of radius 2 and 1.}
  \label{fig:scaling_method}
\end{figure}


%Crossover point for array vs.\ tree, by dimension.

%Memory is obviously linear.


%we can run Bridson's code, available online compare saturation in 5d or so




==> smooth_alg.tex <==
\begin{algorithm}
  \Caption{Two-spoke.}{}
  \label{alg:trim_step_blue_noise}
  \begin{algorithmic} [1]
    \REQUIRE line spoke $\linespoke$ anchored at $a$ for sample $\sample$
    \ENSURE uncovered segment of trimmed spoke $\linespokeprime$    
    \IF{Trim anchor point($a$) = empty}
	\STATE inrement($reject$)
      \RETURN\ empty
    \ENDIF
    \STATE $\linespokeprime \leftarrow$ Trim anchored segment($\linespoke$) \pcomment not empty
    \IF{skip\_trimmed\_spoke AND was\_trimmed(\linespokeprime) 
		\STATE increment($reject$)
			\IF{$reject=6$}
			  \STATE skip\_trimmed\_spoke $\leftarrow$ false
			  \STATE $reject \leftarrow 0$
			\ENDIF
			\RETURN\ empty
  \ENDIF
    \IF{is\_short(\linespokeprime)
	\STATE increment($reject$)
	\RETURN\ empty
  \ENDIF
  \STATE $reject \leftarrow 0$
  \RETURN \linespokeprime
  \end{algorithmic}
\end{algorithm}


==> spectra_d_fig.tex <==
% two columns of power and anisotropy
\begin{figure}[tbh]
\centering

     \rotatebox{90}{$d=2$}
     \includegraphics[width=0.46\linewidth]{figs/spectral_analysis/power-placeholder.jpg}
     \includegraphics[width=0.46\linewidth]{figs/spectral_analysis/anisotropy-placeholder.jpg}

\vspace{10pt}

     \rotatebox{90}{$d=6$}
     \includegraphics[width=0.46\linewidth]{figs/spectral_analysis/power-placeholder.jpg}
     \includegraphics[width=0.46\linewidth]{figs/spectral_analysis/anisotropy-placeholder.jpg}

     \rotatebox{90}{$d=20$}
  \subfloat[Power]
  { \label{fig:spectra_power_by_d} 
     \includegraphics[width=0.46\linewidth]{figs/spectral_analysis/power-placeholder.jpg}
  }
  \subfloat[Anisotropy]
  { \label{fig:spectra_anisotropy_by_d} 
     \includegraphics[width=0.46\linewidth]{figs/spectral_analysis/anisotropy-placeholder.jpg}
  }
 \Caption{Power and anisotropy for line-spokes as the dimension increases, for $\hammerlimit = 12.$}{
 \scott{Li-Yi, these are the plots I would need you to generate.  I'm expecting these to turn out quite boring.
If we are going to do RDF by dimension, we can plot multiple curves on a single plot.}
 }
 \label{fig:power_anisotropy_by_d}
 
\end{figure}


==> spectra_line_by_m_fig.tex <==
% arranged in a square so m=12 is directly below Simple MPS
\begin{figure}[tbh]
\centering
  \subfloat[Simple MPS]
  { \label{fig:spectra_mps}
     \includegraphics[width=0.48\linewidth]{figs/spectral_analysis/spectra-placeholder.jpg}
  }
  \subfloat[Line-spokes $\hammerlimit=1$] %1
  { \label{fig:spectra_linespokes_m1_d2} 
     \includegraphics[width=0.48\linewidth]{figs/spectral_analysis/spectra-placeholder.jpg}
  }
  
  \subfloat[Line-spokes $\hammerlimit=12$] %12
  { \label{fig:spectra_linespokes_m12_d2} 
     \includegraphics[width=0.48\linewidth]{figs/spectral_analysis/spectra-placeholder.jpg}
  }
  \subfloat[Line-spokes $\hammerlimit=12^2$] %144
  { \label{fig:spectra_linespokes_m144_d2} 
     \includegraphics[width=0.48\linewidth]{figs/spectral_analysis/spectra-placeholder.jpg}
  }
 \Caption{Spatial and frequency domain properties of MPS and line-spoke distributions with increasing $\hammerlimit$, in $\dimnumber=2.$}
 {
}
 \label{fig:spectra_line_by_m}
 
\end{figure}


==> spectra_methods_fig.tex <==
% arranged in a square so we can read across for degen, or done for k.
\begin{figure}[tbh]
\centering
  \subfloat[Line-spokes]
  { \label{fig:spectra_linespokes_m12_d2_duplicate} % maybe reorganize
     \includegraphics[width=0.48\linewidth]{figs/spectral_analysis/spectra-placeholder.jpg}
  }
  \subfloat[Degenerate line-spokes] 
  { \label{fig:spectra_degenlinespokes_m12_d2} 
     \includegraphics[width=0.48\linewidth]{figs/spectral_analysis/spectra-placeholder.jpg}
  }
  
  \subfloat[Plane-spokes]
  { \label{fig:spectra_planespokes_m12_d2} 
     \includegraphics[width=0.48\linewidth]{figs/spectral_analysis/spectra-placeholder.jpg}
  }
  \subfloat[Degenerate Plane-spokes] %144
  { \label{fig:spectra_degenplanespokes_m12_d2} 
     \includegraphics[width=0.48\linewidth]{figs/spectral_analysis/spectra-placeholder.jpg}
  }
 \Caption{Spatial and frequency domain properties of distributions produced by different methods, for 
 $\hammerlimit = 12$, in $\dimnumber=2.$}
 {
}
 \label{fig:spectra}
 
\end{figure}


==> spectral_analysis_fig.tex <==
\begin{figure}[tbh]
  \centering

  \subfloat[Line Darts]
  {
     \includegraphics[width=1.0\linewidth]{figs/spectral_analysis/line_darts/10000S.pdf} 
  } 
   
  \subfloat[Line Spokes]
  {
     \includegraphics[width=1.0\linewidth]{figs/spectral_analysis/line_spokes/10000S.pdf} 
  } 

  \subfloat[Degenerate Line Spokes]
  {
     \includegraphics[width=1.0\linewidth]{figs/spectral_analysis/degen_line_spokes/10000S.pdf} 
  } 
     

    

 \caption{Spectral analysis for Line Darts and our methods with a number of successive misses $m = 10K$.}
 
 \label{fig:spectral_analysis}
\end{figure}


==> spokes.tex <==
\subsection{Line-Spokes for Traditional Blue Noise}
\label{sec:sampling}
\label{sec:operation}

Our top level algorithm follows.
We initialize the output set with one random sample and put it into the active pool of front points.
When this pool becomes empty our algorithm terminates.
We remove a random sample $\sample$ from the pool and try to generate new samples $\sampleprime$ from random \spokestext{} $\spokesym$ through $\sample$. 
Accepted samples are added to the pool.
We keep throwing \spokestext{} from the same sample until $\hammerlimit=12$ consecutive \spokestext{} failed to generate an acceptable sample.
Our method is summarized in \Cref{alg:spoke}.
%In low dimensions, a $k$-d tree helps.
\nothing{\liyi{(February 7, 2016) These aren't going to help readers.}%liyi
The key subroutines are CollectNeighbors; selecting a random spoke, RandomSpoke;
trimming that spoke, TrimSpoke;
and point sampling from an uncovered interval, RandomSample.
%These are described next.
}%nothing

\input{spoke_alg}

\subsubsection{Spokes}
\label{sec:spoke_darts}

The line of a spoke passes through a sample $\sample$, and the spoke is the interval $\interval$ of distances from $\sample$.
See \Cref{fig:spokes}.
For \linespokesalg, $\interval=[r,2r]$, because the uncovered region starts at $r$ and the extent of the local front we wish to consider is $2r$.
%e.g.\ $2 \rnumber$ as in \bridsonmethod.
Other algorithms use different $\interval$.
A spoke has a distinguished \emph{anchor} point $\anchor \in \interval$ used to select which segment to retain during trimming.

%At one extreme, anchored spokes, we test whether a particular ``anchor'' point of this line is uncovered, then find the 
%At one extreme, we also consider an arc of a great circle around the $d$-dimensional Poisson-disk 

%\input{spokes_new_fig} %\liyi{(February 7, 2016) I moved \Cref{fig:spokes} to \Cref{sec:building_blocks} for better layout and easier reference.}

\subsubsection{CollectNeighbors}
\label{sec:neighbor_collection}

For a sample on the front, for each spoke we trim it by iterating over the nearby samples.
For spoke-darts with spoke extent $2\rnumber$, a sample is a neighbor if its center distance is less than $3\rnumber.$
A key efficiency is to gather all neighbors once \emph{before} any trimming operations.

In our implementation, we have found that using a $k$-d tree saves time in moderate dimensions;
see \Cref{fig:crossover} for the crossover dimension versus exhaustive search.
We maintain a $k$-d tree of the entire point set.
We collect the subtree of neighbors.
We update the tree and subtree as we successfully add new samples.

\subsubsection{RandomSpoke}
\label{sec:randomspoke}
A \linespoketext{} is generated by selecting a line with random orientation, by choosing a point $p$ from the surface of the disk of $\sample$ uniformly by area.
% of the corresponding sample $\sample$, and extended with length $\spokeradius$ away from $\sample$.
%A random \planespoketext{} is generated by selecting the plane containing two such points.
To pick $p$ we use the classical method of Muller~\shortcite{Muller},
based on the observation that the level sets of a $d$-dimensional Gaussian distribution are $d$-spheres.
To pick a vector uniformly by orientation, generate each of the vector's $\dimnumber$ coordinates independently from a normal (Gaussian) distribution. Then linearly scale the vector of coordinates to the disk radius.

\subsubsection{TrimSpoke}
\label{sec:trim}

Trimming a spoke consists of finding some subset of it that is uncovered by extant disks.
The effect of trimming a segment is to subtract out the interval that is covered by each neighbor.
%See \Cref{alg:all_segments} for an efficient $| \neighbors | \log | \neighbors |$ implementation, which gathers all disk-line intersections then computes the depth of each interval between intersections.
This subtraction primitive is efficient in all dimensions.

For overall efficiency, we quickly discard some spokes and spoke segments.
It is acceptable to discard a spoke even if part of it is not covered.
This retains the correctness of the algorithm, and affects the run-time and final distribution characteristics.
The fastest primitive is to determine if a single  \emph{anchor point} $\anchor$ is covered by a disk, since that just involves checking the squared distance between the point and each neighbor.
See Algorithms~\ref{alg:anchored_point}, \ref{alg:anchored_segment} and \ref{alg:trim_blue_noise}.
Retaining just the uncovered segment containing anchor $\anchor$ is considerably faster than finding all uncovered segments.
However, in \Cref{fig:line_spokes}, this means that the next sample will be chosen from the light red subset of the annulus only, and not the bright red portions. 
(This still gives blue noise, but with a  higher peak distribution at distance $r$ than traditional MPS: 4 versus 3.)
%For efficiency we avoid the overhead of keeping track of all of the resultant segments, and only keep the one containing the anchor point $a,$ if any.
%This also avoids wasting time with further searches in the case that the spoke is completely covered, which is common as the algorithm nears termination.
%Many combinations of these heuristics are possible; 
%the ones we found most useful are summarized in 
%\Cref{alg:trim_blue_noise} and \Cref{alg:trim_wheel}.

\input{line_spoke_alg}
%\input{all_segments_alg}

\input{trims_alg}

%\input{anchor_covered}

%\input{plane_spoke_alg}

\subsubsection{RandomSample}
\label{sec:randomsample}
Here we describe how to select a sample point from an uncovered spoke segment.
For blue noise, it is sufficient to pick a sample \emph{uniformly by length} from an uncovered segment.
One might assume that picking a point uniformly by the swept volume, dependent on the dimension, would mimic picking the point uniformly from the annulus around a point,
and generate better quality blue noise. However, we found this detrimental in practice. 
(In \Cref{sec:bridsonexperiments} we see that \bridsonmethod~\cite{Bridson:2007:FPD}  generates worse blue noise than standard MPS algorithms.)
Exploring more sophisticated selection criteria led us to our step and soft blue noise algorithms; see Sections~\ref{sec:stepbluenoise} and \ref{sec:softbluenoise}.

% Dense blue noise: trim with wheels, pick uniformly?




==> trims_alg.tex <==
\begin{algorithm}
  \Caption{TrimSpoke.}{}
  \label{alg:trim_blue_noise}
  \begin{algorithmic} [1]
    \REQUIRE spoke $\linespoke$ anchored at $\anchor$ for sample $\sample$
    \ENSURE  trimmed $\linespokeprime$  with uncovered interval containing $\anchor$
    \IF{TrimAnchor($\anchor,\sample$) not empty}
      \RETURN\ TrimInterval($\linespoke$) \pcomment not empty
    \ENDIF
     \RETURN\ empty
  \end{algorithmic}
\end{algorithm}

